Generalised Unitarity for Dimensionally Regulated Amplitudes

We present a novel set of Feynman rules and generalised unitarity cut-conditions for computing one-loop amplitudes via d-dimensional integrand reduction algorithm. Our algorithm is suited for analytic as well as numerical result, because all ingredients turn out to have a four-dimensional representation. We will apply this formalism to NLO QCD corrections.

==> DiagramCut/5gT1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(0.,17.)(7.,13.5)(0.,){Straight}{0}
\FAProp(0.,10.)(7.,6.5)(0.,){Straight}{0}
\FAProp(0.,3.)(7.,6.5)(0.,){Straight}{0}
\FAProp(20.,15.)(13.,10.)(0.,){Straight}{0}
\FAProp(20.,5.)(13.,10.)(0.,){Straight}{0}
\FAProp(7.,13.5)(7.,6.5)(0.,){Straight}{0}
\FAProp(7.,13.5)(13.,10.)(0.,){Straight}{0}
\FAProp(7.,6.5)(13.,10.)(0.,){Straight}{0}
%
% Vertices 
\FAVert(7.,13.5){0}
\FAVert(7.,6.5){0}
\FAVert(13.,10.){0}
%
% Label for particles
%
\FALabel(3.60138,15.9328)[bl]{$1$}
\FALabel(3.39862,7.56724)[tr]{$2$}
\FALabel(3.60138,4.06724)[tl]{$3$}
\FALabel(16.7756,11.9221)[tl]{$4$}
\FALabel(16.2244,6.92215)[tr]{$5$}
\FALabel(6.18,10.)[r]{$6$}
\FALabel(10.175,12.3929)[bl]{$7$}
\FALabel(10.175,7.60709)[tl]{$8$}
%
\end{feynartspicture}

==> DiagramCut/5gluons.tex <==
\unitlength=1bp%

\begin{feynartspicture}(432,504)(3,3.3)
\FALabel(33.,69.96)[]{\large $3\quad \to\quad 2$}

\FADiagram{T1}
\FAProp(0.,17.)(7.,13.5)(0.,){Straight}{0}
\FAProp(0.,10.)(7.,6.5)(0.,){Straight}{0}
\FAProp(0.,3.)(7.,6.5)(0.,){Straight}{0}
\FAProp(20.,15.)(13.,10.)(0.,){Straight}{0}
\FAProp(20.,5.)(13.,10.)(0.,){Straight}{0}
\FAProp(7.,13.5)(7.,6.5)(0.,){Straight}{0}
\FAProp(7.,13.5)(13.,10.)(0.,){Straight}{0}
\FAProp(7.,6.5)(13.,10.)(0.,){Straight}{0}
\FAVert(7.,13.5){0}
\FAVert(7.,6.5){0}
\FAVert(13.,10.){0}

\FADiagram{T2}
\FAProp(0.,17.)(10.,12.5)(0.,){Straight}{0}
\FAProp(0.,10.)(6.5,6.5)(0.,){Straight}{0}
\FAProp(0.,3.)(6.5,6.5)(0.,){Straight}{0}
\FAProp(20.,15.)(10.,12.5)(0.,){Straight}{0}
\FAProp(20.,5.)(13.5,6.5)(0.,){Straight}{0}
\FAProp(13.5,6.5)(10.,12.5)(0.,){Straight}{0}
\FAProp(13.5,6.5)(6.5,6.5)(0.,){Straight}{0}
\FAProp(10.,12.5)(6.5,6.5)(0.,){Straight}{0}
\FAVert(13.5,6.5){0}
\FAVert(10.,12.5){0}
\FAVert(6.5,6.5){0}

\FADiagram{T3}
\FAProp(0.,17.)(6.,10.)(0.,){Straight}{0}
\FAProp(0.,10.)(6.,10.)(0.,){Straight}{0}
\FAProp(0.,3.)(6.,10.)(0.,){Straight}{0}
\FAProp(20.,15.)(14.,12.)(0.,){Straight}{0}
\FAProp(20.,5.)(14.,8.)(0.,){Straight}{0}
\FAProp(14.,12.)(14.,8.)(0.,){Straight}{0}
\FAProp(14.,12.)(6.,10.)(0.,){Straight}{0}
\FAProp(14.,8.)(6.,10.)(0.,){Straight}{0}
\FAVert(14.,12.){0}
\FAVert(14.,8.){0}
\FAVert(6.,10.){0}

\FADiagram{T4}
\FAProp(0.,17.)(6.5,13.5)(0.,){Straight}{0}
\FAProp(0.,10.)(6.5,6.5)(0.,){Straight}{0}
\FAProp(0.,3.)(6.5,6.5)(0.,){Straight}{0}
\FAProp(20.,15.)(13.5,13.5)(0.,){Straight}{0}
\FAProp(20.,5.)(13.5,6.5)(0.,){Straight}{0}
\FAProp(6.5,13.5)(13.5,13.5)(0.,){Straight}{0}
\FAProp(6.5,13.5)(6.5,6.5)(0.,){Straight}{0}
\FAProp(13.5,13.5)(13.5,6.5)(0.,){Straight}{0}
\FAProp(13.5,6.5)(6.5,6.5)(0.,){Straight}{0}
\FAVert(6.5,13.5){0}
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\FAVert(6.5,6.5){0}

\FADiagram{T5}
\FAProp(0.,17.)(6.,10.)(0.,){Straight}{0}
\FAProp(0.,10.)(6.,10.)(0.,){Straight}{0}
\FAProp(0.,3.)(6.,10.)(0.,){Straight}{0}
\FAProp(20.,15.)(14.,10.)(0.,){Straight}{0}
\FAProp(20.,5.)(14.,10.)(0.,){Straight}{0}
\FAProp(14.,10.)(6.,10.)(0.8,){Straight}{0}
\FAProp(14.,10.)(6.,10.)(-0.8,){Straight}{0}
\FAVert(14.,10.){0}
\FAVert(6.,10.){0}

\FADiagram{}

\FADiagram{}

\FADiagram{}

\FADiagram{}
\end{feynartspicture}



==> DiagramCut/CL123.1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(16.,11.5)(13.5,10.0)(0.,){/Straight}{1}
\FAProp(16.,8.5)(13.5,10.0)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,10.0)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(6.5,6.5)(13.5,10.0)(0.,){/Cycles}{0}
%\FAProp(13.5,13.5)(13.5,6.5)(0.,){/Straight}{1}
%
% Vertices 
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,10.0){0}
%
% Polarizzazioni
%
\FALabel(4.5, 8.9)[]{\tiny $+$}
\FALabel(4.5, 11.1)[]{\tiny $-$}
\FALabel(9.43333, 13.5333)[]{\tiny $+$}
\FALabel(11.7667, 12.3667)[]{\tiny $-$}
\FALabel(11.7667, 7.6333)[]{\tiny $+$}
\FALabel(9.43333, 6.4667)[]{\tiny $-$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$1$}
\FALabel(3.,16.)[]{\tiny$2$}
\FALabel(17.,12.)[]{\tiny$3$}
\FALabel(17.,8.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CL123.2.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(16.,11.5)(13.5,10.0)(0.,){/Straight}{1}
\FAProp(16.,8.5)(13.5,10.0)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,10.0)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(6.5,6.5)(13.5,10.0)(0.,){/Cycles}{0}
%\FAProp(13.5,13.5)(13.5,6.5)(0.,){/Straight}{1}
%
% Vertices 
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,10.0){0}
%
% Polarizzazioni
%
\FALabel(4.5, 8.9)[]{\tiny $-$}
\FALabel(4.5, 11.1)[]{\tiny $+$}
\FALabel(9.43333, 13.5333)[]{\tiny $-$}
\FALabel(11.7667, 12.3667)[]{\tiny $+$}
\FALabel(11.7667, 7.6333)[]{\tiny $-$}
\FALabel(9.43333, 6.4667)[]{\tiny $+$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$1$}
\FALabel(3.,16.)[]{\tiny$2$}
\FALabel(17.,12.)[]{\tiny$3$}
\FALabel(17.,8.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CL123.3.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(16.,11.5)(13.5,10.0)(0.,){/Straight}{1}
\FAProp(16.,8.5)(13.5,10.0)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,10.0)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(6.5,6.5)(13.5,10.0)(0.,){/Cycles}{0}
%\FAProp(13.5,13.5)(13.5,6.5)(0.,){/Straight}{1}
%
% Vertices 
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,10.0){0}
%
% Polarizzazioni
%
\FALabel(4.5, 8.9)[]{\tiny $0$}
\FALabel(4.5, 11.1)[]{\tiny $0$}
\FALabel(9.43333, 13.5333)[]{\tiny $0$}
\FALabel(11.7667, 12.3667)[]{\tiny $0$}
\FALabel(11.7667, 7.6333)[]{\tiny $0$}
\FALabel(9.43333, 6.4667)[]{\tiny $0$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$1$}
\FALabel(3.,16.)[]{\tiny$2$}
\FALabel(17.,12.)[]{\tiny$3$}
\FALabel(17.,8.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CL123.4.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(16.,11.5)(13.5,10.0)(0.,){/Straight}{1}
\FAProp(16.,8.5)(13.5,10.0)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/ScalarDash}{0}
\FAProp(13.5,10.0)(6.5,13.5)(0.,){/ScalarDash}{0}
\FAProp(6.5,6.5)(13.5,10.0)(0.,){/ScalarDash}{0}
%\FAProp(13.5,13.5)(13.5,6.5)(0.,){/Straight}{1}
%
% Vertices 
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,10.0){0}
%
% Polarizzazioni
%
%\FALabel(4.5, 8.9)[]{\tiny $0$}
%\FALabel(4.5, 11.1)[]{\tiny $0$}
%\FALabel(9.43333, 13.5333)[]{\tiny $0$}
%\FALabel(11.7667, 12.3667)[]{\tiny $0$}
%\FALabel(11.7667, 7.6333)[]{\tiny $0$}
%\FALabel(9.43333, 6.4667)[]{\tiny $0$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$1$}
\FALabel(3.,16.)[]{\tiny$2$}
\FALabel(17.,12.)[]{\tiny$3$}
\FALabel(17.,8.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CL1234.1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,13.5)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,13.5)(13.5,6.5)(0.,){/Straight}{1}
%
% Vertices 
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
%
% Cuts
%\FAProp(15.,10.0)(10.,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.0,10.0)(4.5,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.,15.)(10.0,10.)(0.,){/ScalarDash}{0}
%\FAProp(10.,10.)(10.0,4.5)(0.,){/ScalarDash}{0}
%
% Polarizzazioni
\FALabel(11.1,4.5)[]{\tiny $+$}
\FALabel(8.9,4.5)[]{\tiny $-$}
\FALabel(4.5, 8.9)[]{\tiny $+$}
\FALabel(4.5, 11.1)[]{\tiny $-$}
\FALabel(8.9, 15.)[]{\tiny $+$}
\FALabel(11.1, 15.)[]{\tiny $-$}
\FALabel(15., 11.1)[]{\tiny $\pm$}
\FALabel(15., 8.9)[]{\tiny $\mp$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$1$}
\FALabel(3.,16.)[]{\tiny$2$}
\FALabel(17.,16.)[]{\tiny$3$}
\FALabel(17.,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CL1234.2.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,13.5)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,13.5)(13.5,6.5)(0.,){/Straight}{1}
%
% Vertices 
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
%
% Cuts
%\FAProp(15.,10.0)(10.,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.0,10.0)(4.5,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.,15.)(10.0,10.)(0.,){/ScalarDash}{0}
%\FAProp(10.,10.)(10.0,4.5)(0.,){/ScalarDash}{0}
%
% Polarizzazioni
\FALabel(11.1,4.5)[]{\tiny $-$}
\FALabel(8.9,4.5)[]{\tiny $+$}
\FALabel(4.5, 8.9)[]{\tiny $-$}
\FALabel(4.5, 11.1)[]{\tiny $+$}
\FALabel(8.9, 15.)[]{\tiny $-$}
\FALabel(11.1, 15.)[]{\tiny $+$}
\FALabel(15., 11.1)[]{\tiny $\pm$}
\FALabel(15., 8.9)[]{\tiny $\mp$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$1$}
\FALabel(3.,16.)[]{\tiny$2$}
\FALabel(17.,16.)[]{\tiny$3$}
\FALabel(17.,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CL1234.3.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,13.5)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,13.5)(13.5,6.5)(0.,){/Straight}{1}
%
% Vertices 
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
%
% Cuts
%\FAProp(15.,10.0)(10.,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.0,10.0)(4.5,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.,15.)(10.0,10.)(0.,){/ScalarDash}{0}
%\FAProp(10.,10.)(10.0,4.5)(0.,){/ScalarDash}{0}
%
% Polarizzazioni
\FALabel(11.1,4.5)[]{\tiny $0$}
\FALabel(8.9,4.5)[]{\tiny $0$}
\FALabel(4.5, 8.9)[]{\tiny $0$}
\FALabel(4.5, 11.1)[]{\tiny $0$}
\FALabel(8.9, 15.)[]{\tiny $0$}
\FALabel(11.1, 15.)[]{\tiny $0$}
\FALabel(15., 11.1)[]{\tiny $\pm$}
\FALabel(15., 8.9)[]{\tiny $\mp$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$1$}
\FALabel(3.,16.)[]{\tiny$2$}
\FALabel(17.,16.)[]{\tiny$3$}
\FALabel(17.,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CL1234.4.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/ScalarDash}{0}
\FAProp(13.5,13.5)(6.5,13.5)(0.,){/ScalarDash}{0}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){/ScalarDash}{0}
\FAProp(13.5,13.5)(13.5,6.5)(0.,){/Straight}{1}
%
% Vertices 
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
%
% Cuts
%\FAProp(15.,10.0)(10.,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.0,10.0)(4.5,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.,15.)(10.0,10.)(0.,){/ScalarDash}{0}
%\FAProp(10.,10.)(10.0,4.5)(0.,){/ScalarDash}{0}
%
% Polarizzazioni
%\FALabel(11.1,4.5)[]{\tiny $0$}
%\FALabel(8.9,4.5)[]{\tiny $0$}
%\FALabel(4.5, 8.9)[]{\tiny $0$}
%\FALabel(4.5, 11.1)[]{\tiny $0$}
%\FALabel(8.9, 15.)[]{\tiny $0$}
%\FALabel(11.1, 15.)[]{\tiny $0$}
%\FALabel(15., 11.1)[]{\tiny $\pm$}
%\FALabel(15., 8.9)[]{\tiny $\mp$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$1$}
\FALabel(3.,16.)[]{\tiny$2$}
\FALabel(17.,16.)[]{\tiny$3$}
\FALabel(17.,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CL124.1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(7.5,15.)(10.0,13.5)(0.,){/Cycles}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(12.5,15.)(10.0,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(10.0,13.5)(6.5,6.5)(0.,){/Cycles}{0}
%\FAProp(13.5,13.5)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(10.0,13.5)(13.5,6.5)(0.,){/Straight}{1}
%
% Vertices 
\FAVert(10.0,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(10.0,13.5){0}
\FAVert(13.5,6.5){0}
%
% Cuts
%\FAProp(15.,10.0)(10.,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.0,10.0)(4.5,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.,15.)(10.0,10.)(0.,){/ScalarDash}{0}
%\FAProp(10.,10.)(10.0,4.5)(0.,){/ScalarDash}{0}
%
% Polarizzazioni
\FALabel(11.1,4.5)[]{\tiny $+$}
\FALabel(8.9,4.5)[]{\tiny $-$}
%\FALabel(5.26667, 10.0333)[]{\tiny $h_3$}
\FALabel(6.06667, 9.63333)[]{\tiny $+$}
\FALabel(7.23333, 11.9667)[]{\tiny $-$}
%
\FALabel(12.7667, 11.9667)[]{\tiny $+$}
\FALabel(13.9333, 9.63333)[]{\tiny $-$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$1$}
\FALabel(6.5,16.)[]{\tiny$2$}
\FALabel(13.5,16.0)[]{\tiny$3$}
\FALabel(17.,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CL124.2.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(7.5,15.)(10.0,13.5)(0.,){/Cycles}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(12.5,15.)(10.0,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(10.0,13.5)(6.5,6.5)(0.,){/Cycles}{0}
%\FAProp(13.5,13.5)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(10.0,13.5)(13.5,6.5)(0.,){/Straight}{1}
%
% Vertices 
\FAVert(10.0,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(10.0,13.5){0}
\FAVert(13.5,6.5){0}
%
% Cuts
%\FAProp(15.,10.0)(10.,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.0,10.0)(4.5,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.,15.)(10.0,10.)(0.,){/ScalarDash}{0}
%\FAProp(10.,10.)(10.0,4.5)(0.,){/ScalarDash}{0}
%
% Polarizzazioni
\FALabel(11.1,4.5)[]{\tiny $0$}
\FALabel(8.9,4.5)[]{\tiny $0$}
%\FALabel(5.26667, 10.0333)[]{\tiny $h_3$}
\FALabel(6.06667, 9.63333)[]{\tiny $0$}
\FALabel(7.23333, 11.9667)[]{\tiny $0$}
%
\FALabel(12.7667, 11.9667)[]{\tiny $-$}
\FALabel(13.9333, 9.63333)[]{\tiny $+$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$1$}
\FALabel(6.5,16.)[]{\tiny$2$}
\FALabel(13.5,16.0)[]{\tiny$3$}
\FALabel(17.,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CL124.3.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(7.5,15.)(10.0,13.5)(0.,){/Cycles}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(12.5,15.)(10.0,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(10.0,13.5)(6.5,6.5)(0.,){/ScalarDash}{0}
%\FAProp(13.5,13.5)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){/ScalarDash}{0}
\FAProp(10.0,13.5)(13.5,6.5)(0.,){/Straight}{1}
%
% Vertices 
\FAVert(10.0,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(10.0,13.5){0}
\FAVert(13.5,6.5){0}
%
% Cuts
%\FAProp(15.,10.0)(10.,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.0,10.0)(4.5,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.,15.)(10.0,10.)(0.,){/ScalarDash}{0}
%\FAProp(10.,10.)(10.0,4.5)(0.,){/ScalarDash}{0}
%
% Polarizzazioni
%\FALabel(11.1,4.5)[]{\tiny $0$}
%\FALabel(8.9,4.5)[]{\tiny $0$}
%%\FALabel(5.26667, 10.0333)[]{\tiny $h_3$}
%\FALabel(6.06667, 9.63333)[]{\tiny $0$}
%\FALabel(7.23333, 11.9667)[]{\tiny $0$}
%
\FALabel(12.7667, 11.9667)[]{\tiny $-$}
\FALabel(13.9333, 9.63333)[]{\tiny $+$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$1$}
\FALabel(6.5,16.)[]{\tiny$2$}
\FALabel(13.5,16.0)[]{\tiny$3$}
\FALabel(17.,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CL13.1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
\FAProp(4.,11.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(4.,8.5)(0.,){/Cycles}{0}
\FAProp(16.,11.5)(13.5,10.0)(0.,){/Straight}{1}
\FAProp(16.,8.5)(13.5,10.0)(0.,){/Straight}{-1}
%
\FAVert(6.5,10.){0}
\FAVert(13.5,10.0){0}
%
\FALabel(3.1,8.)[]{\tiny$1$}
\FALabel(3.1,12.)[]{\tiny$2$}
\FALabel(17.,12.)[]{\tiny$3$}
\FALabel(17.,8.)[]{\tiny$4$}
%
\FAProp(6.5,10.)(13.5,10.0)(0.8,){/Cycles}{0}
\FAProp(6.5,10.)(13.5,10.0)(-0.8,){/Cycles}{0}
%
\FALabel(11.1,5.0)[]{\tiny $+$}
\FALabel(8.9,5.0)[]{\tiny $-$}
\FALabel(8.9, 14.5)[]{\tiny $+$}
\FALabel(11.1, 14.5)[]{\tiny $-$}
\end{feynartspicture}

==> DiagramCut/CL13.2.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
\FAProp(4.,11.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(4.,8.5)(0.,){/Cycles}{0}
\FAProp(16.,11.5)(13.5,10.0)(0.,){/Straight}{1}
\FAProp(16.,8.5)(13.5,10.0)(0.,){/Straight}{-1}
%
\FAVert(6.5,10.){0}
\FAVert(13.5,10.0){0}
%
\FALabel(3.1,8.)[]{\tiny$1$}
\FALabel(3.1,12.)[]{\tiny$2$}
\FALabel(17.,12.)[]{\tiny$3$}
\FALabel(17.,8.)[]{\tiny$4$}
%
\FAProp(6.5,10.)(13.5,10.0)(0.8,){/Cycles}{0}
\FAProp(6.5,10.)(13.5,10.0)(-0.8,){/Cycles}{0}
%
\FALabel(11.1,5.0)[]{\tiny $0$}
\FALabel(8.9,5.0)[]{\tiny $0$}
\FALabel(8.9, 14.5)[]{\tiny $+$}
\FALabel(11.1, 14.5)[]{\tiny $-$}
\end{feynartspicture}

==> DiagramCut/CL13.3.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
\FAProp(4.,11.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(4.,8.5)(0.,){/Cycles}{0}
\FAProp(16.,11.5)(13.5,10.0)(0.,){/Straight}{1}
\FAProp(16.,8.5)(13.5,10.0)(0.,){/Straight}{-1}
%
\FAVert(6.5,10.){0}
\FAVert(13.5,10.0){0}
%
\FALabel(3.1,8.)[]{\tiny$1$}
\FALabel(3.1,12.)[]{\tiny$2$}
\FALabel(17.,12.)[]{\tiny$3$}
\FALabel(17.,8.)[]{\tiny$4$}
%
\FAProp(6.5,10.)(13.5,10.0)(0.8,){/Cycles}{0}
\FAProp(6.5,10.)(13.5,10.0)(-0.8,){/Cycles}{0}
%
\FALabel(11.1,5.0)[]{\tiny $+$}
\FALabel(8.9,5.0)[]{\tiny $-$}
\FALabel(8.9, 14.5)[]{\tiny $0$}
\FALabel(11.1, 14.5)[]{\tiny $0$}
\end{feynartspicture}

==> DiagramCut/CL13.4.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
\FAProp(4.,11.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(4.,8.5)(0.,){/Cycles}{0}
\FAProp(16.,11.5)(13.5,10.0)(0.,){/Straight}{1}
\FAProp(16.,8.5)(13.5,10.0)(0.,){/Straight}{-1}
%
\FAVert(6.5,10.){0}
\FAVert(13.5,10.0){0}
%
\FALabel(3.1,8.)[]{\tiny$1$}
\FALabel(3.1,12.)[]{\tiny$2$}
\FALabel(17.,12.)[]{\tiny$3$}
\FALabel(17.,8.)[]{\tiny$4$}
%
\FAProp(6.5,10.)(13.5,10.0)(0.8,){/Cycles}{0}
\FAProp(6.5,10.)(13.5,10.0)(-0.8,){/Cycles}{0}
%
\FALabel(11.1,5.0)[]{\tiny $0$}
\FALabel(8.9,5.0)[]{\tiny $0$}
\FALabel(8.9, 14.5)[]{\tiny $0$}
\FALabel(11.1, 14.5)[]{\tiny $0$}
\end{feynartspicture}

==> DiagramCut/CL13.5.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
\FAProp(4.,11.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(4.,8.5)(0.,){/Cycles}{0}
\FAProp(16.,11.5)(13.5,10.0)(0.,){/Straight}{1}
\FAProp(16.,8.5)(13.5,10.0)(0.,){/Straight}{-1}
%
\FAVert(6.5,10.){0}
\FAVert(13.5,10.0){0}
%
\FALabel(3.1,8.)[]{\tiny$1$}
\FALabel(3.1,12.)[]{\tiny$2$}
\FALabel(17.,12.)[]{\tiny$3$}
\FALabel(17.,8.)[]{\tiny$4$}
%
\FAProp(6.5,10.)(13.5,10.0)(0.8,){/ScalarDash}{0}
\FAProp(6.5,10.)(13.5,10.0)(-0.8,){/ScalarDash}{0}
%
%\FALabel(11.1,5.0)[]{\tiny $0$}
%\FALabel(8.9,5.0)[]{\tiny $0$}
%\FALabel(8.9, 14.5)[]{\tiny $0$}
%\FALabel(11.1, 14.5)[]{\tiny $0$}
\end{feynartspicture}

==> DiagramCut/CL134.1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,11.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(4.,8.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(13.5,13.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,13.5)(13.5,6.5)(0.,){/Straight}{1}
%
% Vertices 
%
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\FAVert(6.5,10.){0}
%
%
% Polarizzazioni
\FALabel(10.5667, 6.4667)[]{\tiny $-$}
\FALabel(8.23333, 7.6333)[]{\tiny $+$}
\FALabel(8.23333, 12.3667)[]{\tiny $-$}
\FALabel(10.5667, 13.5333)[]{\tiny $+$}
\FALabel(15., 11.1)[]{\tiny $\pm$}
\FALabel(15., 8.9)[]{\tiny $\mp$}
%
% External legs
%
\FALabel(3.1,8.)[]{\tiny$1$}
\FALabel(3.1,12.)[]{\tiny$2$}
\FALabel(17.,16.)[]{\tiny$3$}
\FALabel(17.,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CL134.2.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,11.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(4.,8.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(13.5,13.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,13.5)(13.5,6.5)(0.,){/Straight}{1}
%
% Vertices 
%
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\FAVert(6.5,10.){0}
%
%
% Polarizzazioni
\FALabel(10.5667, 6.4667)[]{\tiny $+$}
\FALabel(8.23333, 7.6333)[]{\tiny $-$}
\FALabel(8.23333, 12.3667)[]{\tiny $+$}
\FALabel(10.5667, 13.5333)[]{\tiny $-$}
\FALabel(15., 11.1)[]{\tiny $\pm$}
\FALabel(15., 8.9)[]{\tiny $\mp$}
%
% External legs
%
\FALabel(3.1,8.)[]{\tiny$1$}
\FALabel(3.1,12.)[]{\tiny$2$}
\FALabel(17.,16.)[]{\tiny$3$}
\FALabel(17.,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CL134.3.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,11.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(4.,8.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(13.5,13.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,13.5)(13.5,6.5)(0.,){/Straight}{1}
%
% Vertices 
%
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\FAVert(6.5,10.){0}
%
%
% Polarizzazioni
\FALabel(10.5667, 6.4667)[]{\tiny $0$}
\FALabel(8.23333, 7.6333)[]{\tiny $0$}
\FALabel(8.23333, 12.3667)[]{\tiny $+$}
\FALabel(10.5667, 13.5333)[]{\tiny $-$}
\FALabel(15., 11.1)[]{\tiny $\pm$}
\FALabel(15., 8.9)[]{\tiny $\mp$}
%
% External legs
%
\FALabel(3.1,8.)[]{\tiny$1$}
\FALabel(3.1,12.)[]{\tiny$2$}
\FALabel(17.,16.)[]{\tiny$3$}
\FALabel(17.,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CL134.4.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,11.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(4.,8.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(13.5,13.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,13.5)(13.5,6.5)(0.,){/Straight}{1}
%
% Vertices 
%
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\FAVert(6.5,10.){0}
%
%
% Polarizzazioni
\FALabel(10.5667, 6.4667)[]{\tiny $+$}
\FALabel(8.23333, 7.6333)[]{\tiny $-$}
\FALabel(8.23333, 12.3667)[]{\tiny $0$}
\FALabel(10.5667, 13.5333)[]{\tiny $0$}
\FALabel(15., 11.1)[]{\tiny $\pm$}
\FALabel(15., 8.9)[]{\tiny $\mp$}
%
% External legs
%
\FALabel(3.1,8.)[]{\tiny$1$}
\FALabel(3.1,12.)[]{\tiny$2$}
\FALabel(17.,16.)[]{\tiny$3$}
\FALabel(17.,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CL134.5.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,11.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(4.,8.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(13.5,13.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,13.5)(13.5,6.5)(0.,){/Straight}{1}
%
% Vertices 
%
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\FAVert(6.5,10.){0}
%
%
% Polarizzazioni
\FALabel(10.5667, 6.4667)[]{\tiny $0$}
\FALabel(8.23333, 7.6333)[]{\tiny $0$}
\FALabel(8.23333, 12.3667)[]{\tiny $0$}
\FALabel(10.5667, 13.5333)[]{\tiny $0$}
\FALabel(15., 11.1)[]{\tiny $\pm$}
\FALabel(15., 8.9)[]{\tiny $\mp$}
%
% External legs
%
\FALabel(3.1,8.)[]{\tiny$1$}
\FALabel(3.1,12.)[]{\tiny$2$}
\FALabel(17.,16.)[]{\tiny$3$}
\FALabel(17.,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CL134.6.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,11.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(4.,8.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(13.5,13.5)(6.5,10.0)(0.,){/ScalarDash}{0}
\FAProp(6.5,10.0)(13.5,6.5)(0.,){/ScalarDash}{0}
\FAProp(13.5,13.5)(13.5,6.5)(0.,){/Straight}{1}
%
% Vertices 
%
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\FAVert(6.5,10.){0}
%
%
% Polarizzazioni
%\FALabel(10.5667, 6.4667)[]{\tiny $0$}
%\FALabel(8.23333, 7.6333)[]{\tiny $0$}
%\FALabel(8.23333, 12.3667)[]{\tiny $0$}
%\FALabel(10.5667, 13.5333)[]{\tiny $0$}
\FALabel(15., 11.1)[]{\tiny $\pm$}
\FALabel(15., 8.9)[]{\tiny $\mp$}
%
% External legs
%
\FALabel(3.1,8.)[]{\tiny$1$}
\FALabel(3.1,12.)[]{\tiny$2$}
\FALabel(17.,16.)[]{\tiny$3$}
\FALabel(17.,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CL234.1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(7.5,5.)(10.,6.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(12.5,5.)(10.0,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(6.5,13.5)(10.0,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,13.5)(6.5,13.5)(0.,){/Cycles}{0}
%\FAProp(6.5,6.5)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,13.5)(10.0,6.5)(0.,){/Straight}{1}
%
% Vertices 
%\FAVert(6.5,13.5){0}
\FAVert(6.5,13.5){0}
\FAVert(13.5,13.5){0}
\FAVert(10.0,6.5){0}
%
%
% Polarizzazioni
%\FALabel(11.1,4.5)[]{\tiny $h_1$}
%\FALabel(8.9,4.5)[]{\tiny $h_2$}
\FALabel(8.9, 15.)[]{\tiny $+$}
\FALabel(11.1, 15.)[]{\tiny $-$}
\FALabel(13.9333, 10.3667)[]{\tiny $+$}
\FALabel(12.7667, 8.03333)[]{\tiny $-$}
%
\FALabel(6.0667, 10.3667)[]{\tiny $+$}
\FALabel(7.2333, 8.03333)[]{\tiny $+$}
%
% External legs
%
\FALabel(6.5,4.)[]{\tiny$1$}
\FALabel(3.,16.)[]{\tiny$2$}
\FALabel(17.,16.)[]{\tiny$3$}
\FALabel(13.5,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CL234.2.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(7.5,5.)(10.,6.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(12.5,5.)(10.0,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(6.5,13.5)(10.0,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,13.5)(6.5,13.5)(0.,){/Cycles}{0}
%\FAProp(6.5,6.5)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,13.5)(10.0,6.5)(0.,){/Straight}{1}
%
% Vertices 
%\FAVert(6.5,13.5){0}
\FAVert(6.5,13.5){0}
\FAVert(13.5,13.5){0}
\FAVert(10.0,6.5){0}
%
%
% Polarizzazioni
%\FALabel(11.1,4.5)[]{\tiny $h_1$}
%\FALabel(8.9,4.5)[]{\tiny $h_2$}
\FALabel(8.9, 15.)[]{\tiny $0$}
\FALabel(11.1, 15.)[]{\tiny $0$}
\FALabel(13.9333, 10.3667)[]{\tiny $-$}
\FALabel(12.7667, 8.03333)[]{\tiny $+$}
%
\FALabel(6.0667, 10.3667)[]{\tiny $0$}
\FALabel(7.2333, 8.03333)[]{\tiny $0$}
%
% External legs
%
\FALabel(6.5,4.)[]{\tiny$1$}
\FALabel(3.,16.)[]{\tiny$2$}
\FALabel(17.,16.)[]{\tiny$3$}
\FALabel(13.5,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CL234.3.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(7.5,5.)(10.,6.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(12.5,5.)(10.0,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(6.5,13.5)(10.0,6.5)(0.,){/ScalarDash}{0}
\FAProp(13.5,13.5)(6.5,13.5)(0.,){/ScalarDash}{0}
%\FAProp(6.5,6.5)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,13.5)(10.0,6.5)(0.,){/Straight}{1}
%
% Vertices 
%\FAVert(6.5,13.5){0}
\FAVert(6.5,13.5){0}
\FAVert(13.5,13.5){0}
\FAVert(10.0,6.5){0}
%
%
% Polarizzazioni
%\FALabel(11.1,4.5)[]{\tiny $h_1$}
%\FALabel(8.9,4.5)[]{\tiny $h_2$}
%\FALabel(8.9, 15.)[]{\tiny $0$}
%\FALabel(11.1, 15.)[]{\tiny $0$}
\FALabel(13.9333, 10.3667)[]{\tiny $-$}
\FALabel(12.7667, 8.03333)[]{\tiny $+$}
%
%\FALabel(6.0667, 10.3667)[]{\tiny $0$}
%FALabel(7.2333, 8.03333)[]{\tiny $0$}
%
% External legs
%
\FALabel(6.5,4.)[]{\tiny$1$}
\FALabel(3.,16.)[]{\tiny$2$}
\FALabel(17.,16.)[]{\tiny$3$}
\FALabel(13.5,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CL24.1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
\FAProp(7.5,15.)(10.0,13.5)(0.,){/Cycles}{0}
\FAProp(12.5,15.)(10.0,13.5)(0.,){/Straight}{1}
\FAProp(7.5,5.)(10.,6.5)(0.,){/Cycles}{0}
\FAProp(12.5,5.)(10.0,6.5)(0.,){/Straight}{-1}
%
\FAVert(10.0,13.5){0}
\FAVert(10.0,6.5){0}
%
\FALabel(6.5,16.)[]{\tiny$2$}
\FALabel(13.5,16.0)[]{\tiny$3$}
\FALabel(6.5,4.)[]{\tiny$1$}
\FALabel(13.5,4.)[]{\tiny$4$}
%
\FAProp(10.0,6.5)(10.0,13.5)(0.8,){/Straight}{-1}
\FAProp(10.0,6.5)(10.0,13.5)(-0.8,){/Cycles}{0}
%
\FALabel(5.0, 8.9)[]{\tiny $+$}
\FALabel(5.0, 11.1)[]{\tiny $-$}
\FALabel(14.5, 11.1)[]{\tiny $+$}
\FALabel(14.5, 8.9)[]{\tiny $-$}
%
\end{feynartspicture}

==> DiagramCut/CL24.2.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
\FAProp(7.5,15.)(10.0,13.5)(0.,){/Cycles}{0}
\FAProp(12.5,15.)(10.0,13.5)(0.,){/Straight}{1}
\FAProp(7.5,5.)(10.,6.5)(0.,){/Cycles}{0}
\FAProp(12.5,5.)(10.0,6.5)(0.,){/Straight}{-1}
%
\FAVert(10.0,13.5){0}
\FAVert(10.0,6.5){0}
%
\FALabel(6.5,16.)[]{\tiny$2$}
\FALabel(13.5,16.0)[]{\tiny$3$}
\FALabel(6.5,4.)[]{\tiny$1$}
\FALabel(13.5,4.)[]{\tiny$4$}
%
\FAProp(10.0,6.5)(10.0,13.5)(0.8,){/Straight}{-1}
\FAProp(10.0,6.5)(10.0,13.5)(-0.8,){/Cycles}{0}
%
\FALabel(5.0, 8.9)[]{\tiny $0$}
\FALabel(5.0, 11.1)[]{\tiny $0$}
\FALabel(14.5, 11.1)[]{\tiny $+$}
\FALabel(14.5, 8.9)[]{\tiny $-$}
%
\end{feynartspicture}

==> DiagramCut/CL24.3.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
\FAProp(7.5,15.)(10.0,13.5)(0.,){/Cycles}{0}
\FAProp(12.5,15.)(10.0,13.5)(0.,){/Straight}{1}
\FAProp(7.5,5.)(10.,6.5)(0.,){/Cycles}{0}
\FAProp(12.5,5.)(10.0,6.5)(0.,){/Straight}{-1}
%
\FAVert(10.0,13.5){0}
\FAVert(10.0,6.5){0}
%
\FALabel(6.5,16.)[]{\tiny$2$}
\FALabel(13.5,16.0)[]{\tiny$3$}
\FALabel(6.5,4.)[]{\tiny$1$}
\FALabel(13.5,4.)[]{\tiny$4$}
%
\FAProp(10.0,6.5)(10.0,13.5)(0.8,){/Straight}{-1}
\FAProp(10.0,6.5)(10.0,13.5)(-0.8,){/Cycles}{0}
%
\FALabel(5.0, 8.9)[]{\tiny $0$}
\FALabel(5.0, 11.1)[]{\tiny $0$}
\FALabel(14.5, 11.1)[]{\tiny $-$}
\FALabel(14.5, 8.9)[]{\tiny $+$}
%
\end{feynartspicture}

==> DiagramCut/CL24.4.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
\FAProp(7.5,15.)(10.0,13.5)(0.,){/Cycles}{0}
\FAProp(12.5,15.)(10.0,13.5)(0.,){/Straight}{1}
\FAProp(7.5,5.)(10.,6.5)(0.,){/Cycles}{0}
\FAProp(12.5,5.)(10.0,6.5)(0.,){/Straight}{-1}
%
\FAVert(10.0,13.5){0}
\FAVert(10.0,6.5){0}
%
\FALabel(6.5,16.)[]{\tiny$2$}
\FALabel(13.5,16.0)[]{\tiny$3$}
\FALabel(6.5,4.)[]{\tiny$1$}
\FALabel(13.5,4.)[]{\tiny$4$}
%
\FAProp(10.0,6.5)(10.0,13.5)(0.8,){/Straight}{-1}
\FAProp(10.0,6.5)(10.0,13.5)(-0.8,){/ScalarDash}{0}
%
%\FALabel(5.0, 8.9)[]{\tiny $0$}
%\FALabel(5.0, 11.1)[]{\tiny $0$}
\FALabel(14.5, 11.1)[]{\tiny $-$}
\FALabel(14.5, 8.9)[]{\tiny $+$}
%
\end{feynartspicture}

==> DiagramCut/CR123.1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(16.,11.5)(13.5,10.0)(0.,){/Straight}{1}
\FAProp(16.,8.5)(13.5,10.0)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/Straight}{1}
\FAProp(13.5,10.0)(6.5,13.5)(0.,){/Straight}{1}
\FAProp(6.5,6.5)(13.5,10.0)(0.,){/Straight}{1}
%
% Vertices 
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,10.0){0}
%
% Polarizzazioni
%
\FALabel(4.5, 8.9)[]{\tiny $-$}
\FALabel(4.5, 11.1)[]{\tiny $+$}
\FALabel(9.43333, 13.5333)[]{\tiny $-$}
\FALabel(11.7667, 12.3667)[]{\tiny $+$}
\FALabel(11.7667, 7.6333)[]{\tiny $-$}
\FALabel(9.43333, 6.4667)[]{\tiny $+$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$1$}
\FALabel(3.,16.)[]{\tiny$2$}
\FALabel(17.,12.)[]{\tiny$3$}
\FALabel(17.,8.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CR123.2.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(16.,11.5)(13.5,10.0)(0.,){/Straight}{1}
\FAProp(16.,8.5)(13.5,10.0)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/Straight}{1}
\FAProp(13.5,10.0)(6.5,13.5)(0.,){/Straight}{1}
\FAProp(6.5,6.5)(13.5,10.0)(0.,){/Straight}{1}
%
% Vertices 
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,10.0){0}
%
% Polarizzazioni
%
\FALabel(4.5, 8.9)[]{\tiny $+$}
\FALabel(4.5, 11.1)[]{\tiny $-$}
\FALabel(9.43333, 13.5333)[]{\tiny $+$}
\FALabel(11.7667, 12.3667)[]{\tiny $-$}
\FALabel(11.7667, 7.6333)[]{\tiny $+$}
\FALabel(9.43333, 6.4667)[]{\tiny $-$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$1$}
\FALabel(3.,16.)[]{\tiny$2$}
\FALabel(17.,12.)[]{\tiny$3$}
\FALabel(17.,8.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CR1234.1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/Straight}{1}
\FAProp(13.5,13.5)(6.5,13.5)(0.,){/Straight}{1}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){/Straight}{1}
\FAProp(13.5,6.5)(13.5,13.5)(0.,){/Cycles}{0}
%
% Vertices 
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
%
% Cuts
%\FAProp(15.,10.0)(10.,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.0,10.0)(4.5,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.,15.)(10.0,10.)(0.,){/ScalarDash}{0}
%\FAProp(10.,10.)(10.0,4.5)(0.,){/ScalarDash}{0}
%
% Polarizzazioni
\FALabel(11.1,4.5)[]{\tiny $-$}
\FALabel(8.9,4.5)[]{\tiny $+$}
\FALabel(4.5, 8.9)[]{\tiny $\mp$}
\FALabel(4.5, 11.1)[]{\tiny $\pm$}
\FALabel(8.9, 15.)[]{\tiny $-$}
\FALabel(11.1, 15.)[]{\tiny $+$}
\FALabel(15., 11.1)[]{\tiny $-$}
\FALabel(15., 8.9)[]{\tiny $+$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$1$}
\FALabel(3.,16.)[]{\tiny$2$}
\FALabel(17.,16.)[]{\tiny$3$}
\FALabel(17.,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CR1234.2.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/Straight}{1}
\FAProp(13.5,13.5)(6.5,13.5)(0.,){/Straight}{1}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){/Straight}{1}
\FAProp(13.5,6.5)(13.5,13.5)(0.,){/Cycles}{0}
%
% Vertices 
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
%
% Cuts
%\FAProp(15.,10.0)(10.,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.0,10.0)(4.5,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.,15.)(10.0,10.)(0.,){/ScalarDash}{0}
%\FAProp(10.,10.)(10.0,4.5)(0.,){/ScalarDash}{0}
%
% Polarizzazioni
\FALabel(11.1,4.5)[]{\tiny $+$}
\FALabel(8.9,4.5)[]{\tiny $-$}
\FALabel(4.5, 8.9)[]{\tiny $\mp$}
\FALabel(4.5, 11.1)[]{\tiny $\pm$}
\FALabel(8.9, 15.)[]{\tiny $+$}
\FALabel(11.1, 15.)[]{\tiny $-$}
\FALabel(15., 11.1)[]{\tiny $0$}
\FALabel(15., 8.9)[]{\tiny $0$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$1$}
\FALabel(3.,16.)[]{\tiny$2$}
\FALabel(17.,16.)[]{\tiny$3$}
\FALabel(17.,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CR1234.3.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/Straight}{1}
\FAProp(13.5,13.5)(6.5,13.5)(0.,){/Straight}{1}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){/Straight}{1}
\FAProp(13.5,6.5)(13.5,13.5)(0.,){/ScalarDash}{0}
%
% Vertices 
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
%
% Cuts
%\FAProp(15.,10.0)(10.,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.0,10.0)(4.5,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.,15.)(10.0,10.)(0.,){/ScalarDash}{0}
%\FAProp(10.,10.)(10.0,4.5)(0.,){/ScalarDash}{0}
%
% Polarizzazioni
\FALabel(11.1,4.5)[]{\tiny $+$}
\FALabel(8.9,4.5)[]{\tiny $-$}
\FALabel(4.5, 8.9)[]{\tiny $\mp$}
\FALabel(4.5, 11.1)[]{\tiny $\pm$}
\FALabel(8.9, 15.)[]{\tiny $+$}
\FALabel(11.1, 15.)[]{\tiny $-$}
%\FALabel(15., 11.1)[]{\tiny $0$}
%\FALabel(15., 8.9)[]%\tiny $0$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$1$}
\FALabel(3.,16.)[]{\tiny$2$}
\FALabel(17.,16.)[]{\tiny$3$}
\FALabel(17.,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CR124.1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(7.5,15.)(10.0,13.5)(0.,){/Cycles}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(12.5,15.)(10.0,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(10.0,13.5)(6.5,6.5)(0.,){/Straight}{1}
%\FAProp(13.5,13.5)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){/Straight}{1}
\FAProp(13.5,6.5)(10.0,13.5)(0.,){/Cycles}{0}
%
% Vertices 
\FAVert(10.0,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(10.0,13.5){0}
\FAVert(13.5,6.5){0}
%
% Cuts
%\FAProp(15.,10.0)(10.,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.0,10.0)(4.5,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.,15.)(10.0,10.)(0.,){/ScalarDash}{0}
%\FAProp(10.,10.)(10.0,4.5)(0.,){/ScalarDash}{0}
%
% Polarizzazioni
\FALabel(11.1,4.5)[]{\tiny $-$}
\FALabel(8.9,4.5)[]{\tiny $+$}
%\FALabel(5.26667, 10.0333)[]{\tiny $h_3$}
\FALabel(6.06667, 9.63333)[]{\tiny $-$}
\FALabel(7.23333, 11.9667)[]{\tiny $+$}
%
\FALabel(12.7667, 11.9667)[]{\tiny $-$}
\FALabel(13.9333, 9.63333)[]{\tiny $+$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$1$}
\FALabel(6.5,16.)[]{\tiny$2$}
\FALabel(13.5,16.0)[]{\tiny$3$}
\FALabel(17.,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CR124.2.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(7.5,15.)(10.0,13.5)(0.,){/Cycles}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(12.5,15.)(10.0,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(10.0,13.5)(6.5,6.5)(0.,){/Straight}{1}
%\FAProp(13.5,13.5)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){/Straight}{1}
\FAProp(13.5,6.5)(10.0,13.5)(0.,){/Cycles}{0}
%
% Vertices 
\FAVert(10.0,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(10.0,13.5){0}
\FAVert(13.5,6.5){0}
%
% Cuts
%\FAProp(15.,10.0)(10.,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.0,10.0)(4.5,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.,15.)(10.0,10.)(0.,){/ScalarDash}{0}
%\FAProp(10.,10.)(10.0,4.5)(0.,){/ScalarDash}{0}
%
% Polarizzazioni
\FALabel(11.1,4.5)[]{\tiny $+$}
\FALabel(8.9,4.5)[]{\tiny $-$}
%\FALabel(5.26667, 10.0333)[]{\tiny $h_3$}
\FALabel(6.06667, 9.63333)[]{\tiny $+$}
\FALabel(7.23333, 11.9667)[]{\tiny $-$}
%
\FALabel(12.7667, 11.9667)[]{\tiny $0$}
\FALabel(13.9333, 9.63333)[]{\tiny $0$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$1$}
\FALabel(6.5,16.)[]{\tiny$2$}
\FALabel(13.5,16.0)[]{\tiny$3$}
\FALabel(17.,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CR124.3.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(7.5,15.)(10.0,13.5)(0.,){/Cycles}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(12.5,15.)(10.0,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(10.0,13.5)(6.5,6.5)(0.,){/Straight}{1}
%\FAProp(13.5,13.5)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){/Straight}{1}
\FAProp(13.5,6.5)(10.0,13.5)(0.,){/ScalarDash}{0}
%
% Vertices 
\FAVert(10.0,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(10.0,13.5){0}
\FAVert(13.5,6.5){0}
%
% Cuts
%\FAProp(15.,10.0)(10.,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.0,10.0)(4.5,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.,15.)(10.0,10.)(0.,){/ScalarDash}{0}
%\FAProp(10.,10.)(10.0,4.5)(0.,){/ScalarDash}{0}
%
% Polarizzazioni
\FALabel(11.1,4.5)[]{\tiny $+$}
\FALabel(8.9,4.5)[]{\tiny $-$}
%\FALabel(5.26667, 10.0333)[]{\tiny $h_3$}
\FALabel(6.06667, 9.63333)[]{\tiny $+$}
\FALabel(7.23333, 11.9667)[]{\tiny $-$}
%
%\FALabel(12.7667, 11.9667)[]{\tiny $0$}
%\FALabel(13.9333, 9.63333)[]{\tiny $0$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$1$}
\FALabel(6.5,16.)[]{\tiny$2$}
\FALabel(13.5,16.0)[]{\tiny$3$}
\FALabel(17.,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CR13.1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
\FAProp(4.,11.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(4.,8.5)(0.,){/Cycles}{0}
\FAProp(16.,11.5)(13.5,10.0)(0.,){/Straight}{1}
\FAProp(16.,8.5)(13.5,10.0)(0.,){/Straight}{-1}
%
\FAVert(6.5,10.){0}
\FAVert(13.5,10.0){0}
%
\FALabel(3.1,8.)[]{\tiny$1$}
\FALabel(3.1,12.)[]{\tiny$2$}
\FALabel(17.,12.)[]{\tiny$3$}
\FALabel(17.,8.)[]{\tiny$4$}
%
\FAProp(6.5,10.)(13.5,10.0)(0.8,){/Straight}{1}
\FAProp(6.5,10.)(13.5,10.0)(-0.8,){/Straight}{-1}
%
\FALabel(11.1,5.0)[]{\tiny $-$}
\FALabel(8.9,5.0)[]{\tiny $+$}
\FALabel(8.9, 14.5)[]{\tiny $-$}
\FALabel(11.1, 14.5)[]{\tiny $+$}
\end{feynartspicture}

==> DiagramCut/CR134.1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,11.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(4.,8.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(13.5,13.5)(6.5,10.0)(0.,){/Straight}{1}
\FAProp(6.5,10.0)(13.5,6.5)(0.,){/Straight}{1}
\FAProp(13.5,6.5)(13.5,13.5)(0.,){/Cycles}{0}
%
% Vertices 
%
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\FAVert(6.5,10.){0}
%
%
% Polarizzazioni
\FALabel(10.5667, 6.4667)[]{\tiny $-$}
\FALabel(8.23333, 7.6333)[]{\tiny $+$}
\FALabel(8.23333, 12.3667)[]{\tiny $-$}
\FALabel(10.5667, 13.5333)[]{\tiny $+$}
\FALabel(15., 11.1)[]{\tiny $\pm$}
\FALabel(15., 8.9)[]{\tiny $\mp$}
%
% External legs
%
\FALabel(3.1,8.)[]{\tiny$1$}
\FALabel(3.1,12.)[]{\tiny$2$}
\FALabel(17.,16.)[]{\tiny$3$}
\FALabel(17.,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CR134.2.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,11.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(4.,8.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(13.5,13.5)(6.5,10.0)(0.,){/Straight}{1}
\FAProp(6.5,10.0)(13.5,6.5)(0.,){/Straight}{1}
\FAProp(13.5,6.5)(13.5,13.5)(0.,){/Cycles}{0}
%
% Vertices 
%
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\FAVert(6.5,10.){0}
%
%
% Polarizzazioni
\FALabel(10.5667, 6.4667)[]{\tiny $+$}
\FALabel(8.23333, 7.6333)[]{\tiny $-$}
\FALabel(8.23333, 12.3667)[]{\tiny $+$}
\FALabel(10.5667, 13.5333)[]{\tiny $-$}
\FALabel(15., 11.1)[]{\tiny $+$}
\FALabel(15., 8.9)[]{\tiny $-$}
%
% External legs
%
\FALabel(3.1,8.)[]{\tiny$1$}
\FALabel(3.1,12.)[]{\tiny$2$}
\FALabel(17.,16.)[]{\tiny$3$}
\FALabel(17.,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CR134.3.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,11.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(4.,8.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(13.5,13.5)(6.5,10.0)(0.,){/Straight}{1}
\FAProp(6.5,10.0)(13.5,6.5)(0.,){/Straight}{1}
\FAProp(13.5,6.5)(13.5,13.5)(0.,){/ScalarDash}{0}
%
% Vertices 
%
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\FAVert(6.5,10.){0}
%
%
% Polarizzazioni
\FALabel(10.5667, 6.4667)[]{\tiny $\mp$}
\FALabel(8.23333, 7.6333)[]{\tiny $\pm$}
\FALabel(8.23333, 12.3667)[]{\tiny $\mp$}
\FALabel(10.5667, 13.5333)[]{\tiny $\pm$}
%\FALabel(15., 11.1)[]{\tiny $h_5$}
%\FALabel(15., 8.9)[]{\tiny $h_6$}
%
% External legs
%
\FALabel(3.1,8.)[]{\tiny$1$}
\FALabel(3.1,12.)[]{\tiny$2$}
\FALabel(17.,16.)[]{\tiny$3$}
\FALabel(17.,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CR134.4.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,11.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(4.,8.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(13.5,13.5)(6.5,10.0)(0.,){/Straight}{1}
\FAProp(6.5,10.0)(13.5,6.5)(0.,){/Straight}{1}
\FAProp(13.5,6.5)(13.5,13.5)(0.,){/Cycles}{0}
%
% Vertices 
%
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\FAVert(6.5,10.){0}
%
%
% Polarizzazioni
\FALabel(10.5667, 6.4667)[]{\tiny $-$}
\FALabel(8.23333, 7.6333)[]{\tiny $+$}
\FALabel(8.23333, 12.3667)[]{\tiny $-$}
\FALabel(10.5667, 13.5333)[]{\tiny $+$}
\FALabel(15., 11.1)[]{\tiny $0$}
\FALabel(15., 8.9)[]{\tiny $0$}
%
% External legs
%
\FALabel(3.1,8.)[]{\tiny$1$}
\FALabel(3.1,12.)[]{\tiny$2$}
\FALabel(17.,16.)[]{\tiny$3$}
\FALabel(17.,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CR134.5.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,11.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(4.,8.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(13.5,13.5)(6.5,10.0)(0.,){/Straight}{1}
\FAProp(6.5,10.0)(13.5,6.5)(0.,){/Straight}{1}
\FAProp(13.5,6.5)(13.5,13.5)(0.,){/Cycles}{0}
%
% Vertices 
%
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\FAVert(6.5,10.){0}
%
%
% Polarizzazioni
\FALabel(10.5667, 6.4667)[]{\tiny $\mp$}
\FALabel(8.23333, 7.6333)[]{\tiny $\pm$}
\FALabel(8.23333, 12.3667)[]{\tiny $\mp$}
\FALabel(10.5667, 13.5333)[]{\tiny $\pm$}
\FALabel(15., 11.1)[]{\tiny $0$}
\FALabel(15., 8.9)[]{\tiny $0$}
%
% External legs
%
\FALabel(3.1,8.)[]{\tiny$1$}
\FALabel(3.1,12.)[]{\tiny$2$}
\FALabel(17.,16.)[]{\tiny$3$}
\FALabel(17.,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CR234.1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(7.5,5.)(10.,6.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(12.5,5.)(10.0,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(6.5,13.5)(10.0,6.5)(0.,){/Straight}{1}
\FAProp(13.5,13.5)(6.5,13.5)(0.,){/Straight}{1}
\FAProp(10.0,6.5)(13.5,13.5)(0.,){/Cycles}{0}
%
% Vertices 
%\FAVert(6.5,13.5){0}
\FAVert(6.5,13.5){0}
\FAVert(13.5,13.5){0}
\FAVert(10.0,6.5){0}
%
%
% Polarizzazioni
%\FALabel(11.1,4.5)[]{\tiny $h_1$}
%\FALabel(8.9,4.5)[]{\tiny $h_2$}
\FALabel(8.9, 15.)[]{\tiny $-$}
\FALabel(11.1, 15.)[]{\tiny $+$}
\FALabel(13.9333, 10.3667)[]{\tiny $-$}
\FALabel(12.7667, 8.03333)[]{\tiny $+$}
%
\FALabel(6.0667, 10.3667)[]{\tiny $+$}
\FALabel(7.2333, 8.03333)[]{\tiny $-$}
%
% External legs
%
\FALabel(6.5,4.)[]{\tiny$1$}
\FALabel(3.,16.)[]{\tiny$2$}
\FALabel(17.,16.)[]{\tiny$3$}
\FALabel(13.5,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CR234.2.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(7.5,5.)(10.,6.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(12.5,5.)(10.0,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(6.5,13.5)(10.0,6.5)(0.,){/Straight}{1}
\FAProp(13.5,13.5)(6.5,13.5)(0.,){/Straight}{1}
\FAProp(10.0,6.5)(13.5,13.5)(0.,){/Cycles}{0}
%
% Vertices 
%\FAVert(6.5,13.5){0}
\FAVert(6.5,13.5){0}
\FAVert(13.5,13.5){0}
\FAVert(10.0,6.5){0}
%
%
% Polarizzazioni
%\FALabel(11.1,4.5)[]{\tiny $h_1$}
%\FALabel(8.9,4.5)[]{\tiny $h_2$}
\FALabel(8.9, 15.)[]{\tiny $+$}
\FALabel(11.1, 15.)[]{\tiny $-$}
\FALabel(13.9333, 10.3667)[]{\tiny $0$}
\FALabel(12.7667, 8.03333)[]{\tiny $0$}
%
\FALabel(6.0667, 10.3667)[]{\tiny $-$}
\FALabel(7.2333, 8.03333)[]{\tiny $+$}
%
% External legs
%
\FALabel(6.5,4.)[]{\tiny$1$}
\FALabel(3.,16.)[]{\tiny$2$}
\FALabel(17.,16.)[]{\tiny$3$}
\FALabel(13.5,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CR234.3.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(7.5,5.)(10.,6.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(12.5,5.)(10.0,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(6.5,13.5)(10.0,6.5)(0.,){/Straight}{1}
\FAProp(13.5,13.5)(6.5,13.5)(0.,){/Straight}{1}
\FAProp(10.0,6.5)(13.5,13.5)(0.,){/ScalarDash}{0}
%
% Vertices 
%\FAVert(6.5,13.5){0}
\FAVert(6.5,13.5){0}
\FAVert(13.5,13.5){0}
\FAVert(10.0,6.5){0}
%
%
% Polarizzazioni
%\FALabel(11.1,4.5)[]{\tiny $h_1$}
%\FALabel(8.9,4.5)[]{\tiny $h_2$}
\FALabel(8.9, 15.)[]{\tiny $+$}
\FALabel(11.1, 15.)[]{\tiny $-$}
%\FALabel(13.9333, 10.3667)[]{\tiny $0$}
%\FALabel(12.7667, 8.03333)[]{\tiny $0$}
%
\FALabel(6.0667, 10.3667)[]{\tiny $-$}
\FALabel(7.2333, 8.03333)[]{\tiny $+$}
%
% External legs
%
\FALabel(6.5,4.)[]{\tiny$1$}
\FALabel(3.,16.)[]{\tiny$2$}
\FALabel(17.,16.)[]{\tiny$3$}
\FALabel(13.5,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> DiagramCut/CR24.1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
\FAProp(7.5,15.)(10.0,13.5)(0.,){/Cycles}{0}
\FAProp(12.5,15.)(10.0,13.5)(0.,){/Straight}{1}
\FAProp(7.5,5.)(10.,6.5)(0.,){/Cycles}{0}
\FAProp(12.5,5.)(10.0,6.5)(0.,){/Straight}{-1}
%
\FAVert(10.0,13.5){0}
\FAVert(10.0,6.5){0}
%
\FALabel(6.5,16.)[]{\tiny$2$}
\FALabel(13.5,16.0)[]{\tiny$3$}
\FALabel(6.5,4.)[]{\tiny$1$}
\FALabel(13.5,4.)[]{\tiny$4$}
%
\FAProp(10.0,6.5)(10.0,13.5)(0.8,){/Cycles}{0}
\FAProp(10.0,6.5)(10.0,13.5)(-0.8,){/Straight}{-1}
%
\FALabel(5.0, 8.9)[]{\tiny $-$}
\FALabel(5.0, 11.1)[]{\tiny $+$}
\FALabel(14.5, 11.1)[]{\tiny $-$}
\FALabel(14.5, 8.9)[]{\tiny $+$}
%
\end{feynartspicture}

==> DiagramCut/CR24.2.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
\FAProp(7.5,15.)(10.0,13.5)(0.,){/Cycles}{0}
\FAProp(12.5,15.)(10.0,13.5)(0.,){/Straight}{1}
\FAProp(7.5,5.)(10.,6.5)(0.,){/Cycles}{0}
\FAProp(12.5,5.)(10.0,6.5)(0.,){/Straight}{-1}
%
\FAVert(10.0,13.5){0}
\FAVert(10.0,6.5){0}
%
\FALabel(6.5,16.)[]{\tiny$2$}
\FALabel(13.5,16.0)[]{\tiny$3$}
\FALabel(6.5,4.)[]{\tiny$1$}
\FALabel(13.5,4.)[]{\tiny$4$}
%
\FAProp(10.0,6.5)(10.0,13.5)(0.8,){/Cycles}{0}
\FAProp(10.0,6.5)(10.0,13.5)(-0.8,){/Straight}{-1}
%
\FALabel(5.0, 8.9)[]{\tiny $+$}
\FALabel(5.0, 11.1)[]{\tiny $-$}
\FALabel(14.5, 11.1)[]{\tiny $0$}
\FALabel(14.5, 8.9)[]{\tiny $0$}
%
\end{feynartspicture}

==> DiagramCut/CR24.3.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
\FAProp(7.5,15.)(10.0,13.5)(0.,){/Cycles}{0}
\FAProp(12.5,15.)(10.0,13.5)(0.,){/Straight}{1}
\FAProp(7.5,5.)(10.,6.5)(0.,){/Cycles}{0}
\FAProp(12.5,5.)(10.0,6.5)(0.,){/Straight}{-1}
%
\FAVert(10.0,13.5){0}
\FAVert(10.0,6.5){0}
%
\FALabel(6.5,16.)[]{\tiny$2$}
\FALabel(13.5,16.0)[]{\tiny$3$}
\FALabel(6.5,4.)[]{\tiny$1$}
\FALabel(13.5,4.)[]{\tiny$4$}
%
\FAProp(10.0,6.5)(10.0,13.5)(0.8,){/ScalarDash}{0}
\FAProp(10.0,6.5)(10.0,13.5)(-0.8,){/Straight}{-1}
%
\FALabel(5.0, 8.9)[]{\tiny $+$}
\FALabel(5.0, 11.1)[]{\tiny $-$}
%\FALabel(14.5, 11.1)[]{\tiny $0$}
%\FALabel(14.5, 8.9)[]{\tiny $0$}
%
\end{feynartspicture}

==> DiagramCut/d1.tex <==
\unitlength=1bp%

\begin{feynartspicture}(432,504)(3,3.3)
\FALabel(33.,69.96)[]{\large $4\quad \to\quad 2$}

\FADiagram{T1}

\FADiagram{T2}

\FADiagram{T3}

\FADiagram{T4}

\FADiagram{T5}

\FADiagram{T6}

\FADiagram{}

\FADiagram{}

\FADiagram{}
\end{feynartspicture}



==> DiagramCut/d2.tex <==
\unitlength=1bp%

\begin{feynartspicture}(432,504)(3,3.3)
\FALabel(33.,69.96)[]{\large $3\quad \to\quad 3$}

\FADiagram{T1}

\FADiagram{}

\FADiagram{}

\FADiagram{}

\FADiagram{}

\FADiagram{}

\FADiagram{}

\FADiagram{}

\FADiagram{}
\end{feynartspicture}



==> DiagramCut/d3.tex <==
\unitlength=1bp%

\begin{feynartspicture}(432,504)(3,3.3)
\FALabel(33.,69.96)[]{\large $3\quad \to\quad 3$}

\FADiagram{T1}

\FADiagram{}

\FADiagram{}

\FADiagram{}

\FADiagram{}

\FADiagram{}

\FADiagram{}

\FADiagram{}

\FADiagram{}
\end{feynartspicture}



==> DiagramCut/d4.tex <==
\unitlength=1bp%

\begin{feynartspicture}(432,504)(3,3.3)
\FALabel(33.,69.96)[]{\large $2\quad \to\quad 4$}

\FADiagram{T1}

\FADiagram{}

\FADiagram{}

\FADiagram{}

\FADiagram{}

\FADiagram{}

\FADiagram{}

\FADiagram{}

\FADiagram{}
\end{feynartspicture}



==> DiagramHiggs/C12.1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
\FAProp(7.5,15.)(10.0,13.5)(0.,){/Cycles}{0}
\FAProp(12.5,15.)(10.0,13.5)(0.,){/Cycles}{0}
\FAProp(7.5,5.)(10.,6.5)(0.,){/Cycles}{0}
\FAProp(12.5,5.)(10.0,6.5)(0.,){/ScalarDash}{0}
%
\FAVert(10.0,13.5){0}
\FAVert(10.0,6.5){0}
%
\FALabel(6.5,16.)[]{\tiny$2^+$}
\FALabel(13.5,16.0)[]{\tiny$3^+$}
\FALabel(6.5,4.)[]{\tiny$1^-$}
\FALabel(13.5,4.)[]{\tiny$H$}
%
\FAProp(10.0,6.5)(10.0,13.5)(0.8,){/Cycles}{0}
\FAProp(10.0,6.5)(10.0,13.5)(-0.8,){/Cycles}{0}
%
%\FALabel(5.0, 8.9)[]{\tiny $h_1$}
%\FALabel(5.0, 11.1)[]{\tiny $h_2$}
%\FALabel(14.5, 11.1)[]{\tiny $h_3$}
%\FALabel(14.5, 8.9)[]{\tiny $h_4$}
%
\end{feynartspicture}

==> DiagramHiggs/C12.2.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
\FAProp(7.5,15.)(10.0,13.5)(0.,){/Cycles}{0}
\FAProp(12.5,15.)(10.0,13.5)(0.,){/Cycles}{0}
\FAProp(7.5,5.)(10.,6.5)(0.,){/Cycles}{0}
\FAProp(12.5,5.)(10.0,6.5)(0.,){/ScalarDash}{0}
%
\FAVert(10.0,13.5){0}
\FAVert(10.0,6.5){0}
%
\FALabel(6.5,16.)[]{\tiny$2^+$}
\FALabel(13.5,16.0)[]{\tiny$3^+$}
\FALabel(6.5,4.)[]{\tiny$1^-$}
\FALabel(13.5,4.)[]{\tiny$H$}
%
\FAProp(10.0,6.5)(10.0,13.5)(0.8,){/ScalarDash}{0}
\FAProp(10.0,6.5)(10.0,13.5)(-0.8,){/ScalarDash}{0}
%
%\FALabel(5.0, 8.9)[]{\tiny $h_1$}
%\FALabel(5.0, 11.1)[]{\tiny $h_2$}
%\FALabel(14.5, 11.1)[]{\tiny $h_3$}
%\FALabel(14.5, 8.9)[]{\tiny $h_4$}
%
\end{feynartspicture}

==> DiagramHiggs/C123b.1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(16.,11.5)(13.5,10.0)(0.,){/Cycles}{0}
\FAProp(16.,8.5)(13.5,10.0)(0.,){/ScalarDash}{0}
%
% Internal lines
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,10.0)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(6.5,6.5)(13.5,10.0)(0.,){/Cycles}{0}
%\FAProp(13.5,13.5)(13.5,6.5)(0.,){/Straight}{1}
%
% Vertices 
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,10.0){0}
%
% Polarizzazioni
%
%\FALabel(4.5, 8.9)[]{\tiny $h_1$}
%\FALabel(4.5, 11.1)[]{\tiny $h_2$}
%\FALabel(9.43333, 13.5333)[]{\tiny $h_3$}
%\FALabel(11.7667, 12.3667)[]{\tiny $h_4$}
%\FALabel(11.7667, 7.6333)[]{\tiny $h_5$}
%\FALabel(9.43333, 6.4667)[]{\tiny $h_6$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$3^+$}
\FALabel(3.,16.)[]{\tiny$1^-$}
\FALabel(17.,12.)[]{\tiny$2^+$}
\FALabel(17.,8.)[]{\tiny$H$}
%
\end{feynartspicture}

==> DiagramHiggs/C123b.2.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(16.,11.5)(13.5,10.0)(0.,){/Cycles}{0}
\FAProp(16.,8.5)(13.5,10.0)(0.,){/ScalarDash}{0}
%
% Internal lines
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/ScalarDash}{0}
\FAProp(13.5,10.0)(6.5,13.5)(0.,){/ScalarDash}{0}
\FAProp(6.5,6.5)(13.5,10.0)(0.,){/ScalarDash}{0}
%\FAProp(13.5,13.5)(13.5,6.5)(0.,){/Straight}{1}
%
% Vertices 
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,10.0){0}
%
% Polarizzazioni
%
%\FALabel(4.5, 8.9)[]{\tiny $h_1$}
%\FALabel(4.5, 11.1)[]{\tiny $h_2$}
%\FALabel(9.43333, 13.5333)[]{\tiny $h_3$}
%\FALabel(11.7667, 12.3667)[]{\tiny $h_4$}
%\FALabel(11.7667, 7.6333)[]{\tiny $h_5$}
%\FALabel(9.43333, 6.4667)[]{\tiny $h_6$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$3^+$}
\FALabel(3.,16.)[]{\tiny$1^-$}
\FALabel(17.,12.)[]{\tiny$2^+$}
\FALabel(17.,8.)[]{\tiny$H$}
%
\end{feynartspicture}

==> DiagramHiggs/C123c.1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(16.,11.5)(13.5,10.0)(0.,){/Cycles}{0}
\FAProp(16.,8.5)(13.5,10.0)(0.,){/ScalarDash}{0}
%
% Internal lines
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,10.0)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(6.5,6.5)(13.5,10.0)(0.,){/Cycles}{0}
%\FAProp(13.5,13.5)(13.5,6.5)(0.,){/Straight}{1}
%
% Vertices 
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,10.0){0}
%
% Polarizzazioni
%
%\FALabel(4.5, 8.9)[]{\tiny $h_1$}
%\FALabel(4.5, 11.1)[]{\tiny $h_2$}
%\FALabel(9.43333, 13.5333)[]{\tiny $h_3$}
%\FALabel(11.7667, 12.3667)[]{\tiny $h_4$}
%\FALabel(11.7667, 7.6333)[]{\tiny $h_5$}
%\FALabel(9.43333, 6.4667)[]{\tiny $h_6$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$2^+$}
\FALabel(3.,16.)[]{\tiny$3^+$}
\FALabel(17.,12.)[]{\tiny$1^-$}
\FALabel(17.,8.)[]{\tiny$H$}
%
\end{feynartspicture}

==> DiagramHiggs/C123c.2.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(16.,11.5)(13.5,10.0)(0.,){/Cycles}{0}
\FAProp(16.,8.5)(13.5,10.0)(0.,){/ScalarDash}{0}
%
% Internal lines
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/ScalarDash}{0}
\FAProp(13.5,10.0)(6.5,13.5)(0.,){/ScalarDash}{0}
\FAProp(6.5,6.5)(13.5,10.0)(0.,){/ScalarDash}{0}
%\FAProp(13.5,13.5)(13.5,6.5)(0.,){/Straight}{1}
%
% Vertices 
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,10.0){0}
%
% Polarizzazioni
%
%\FALabel(4.5, 8.9)[]{\tiny $h_1$}
%\FALabel(4.5, 11.1)[]{\tiny $h_2$}
%\FALabel(9.43333, 13.5333)[]{\tiny $h_3$}
%\FALabel(11.7667, 12.3667)[]{\tiny $h_4$}
%\FALabel(11.7667, 7.6333)[]{\tiny $h_5$}
%\FALabel(9.43333, 6.4667)[]{\tiny $h_6$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$2^+$}
\FALabel(3.,16.)[]{\tiny$3^+$}
\FALabel(17.,12.)[]{\tiny$1^-$}
\FALabel(17.,8.)[]{\tiny$H$}
%
\end{feynartspicture}

==> DiagramHiggs/C12H.1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(7.5,15.)(10.0,13.5)(0.,){/Cycles}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(12.5,15.)(10.0,13.5)(0.,){/Cycles}{0}
\FAProp(16.,5.)(13.5,6.5)(0.,){/ScalarDash}{0}
%
% Internal lines
\FAProp(10.0,13.5)(6.5,6.5)(0.,){/Cycles}{0}
%\FAProp(13.5,13.5)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(10.0,13.5)(13.5,6.5)(0.,){/Cycles}{0}
%
% Vertices 
\FAVert(10.0,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(10.0,13.5){0}
\FAVert(13.5,6.5){0}
%
% Cuts
%\FAProp(15.,10.0)(10.,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.0,10.0)(4.5,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.,15.)(10.0,10.)(0.,){/ScalarDash}{0}
%\FAProp(10.,10.)(10.0,4.5)(0.,){/ScalarDash}{0}
%
% Polarizzazioni
%\FALabel(11.1,4.5)[]{\tiny $h_1$}
%\FALabel(8.9,4.5)[]{\tiny $h_2$}
%\FALabel(5.26667, 10.0333)[]{\tiny $h_3$}
%\FALabel(6.06667, 9.63333)[]{\tiny $h_3$}
%\FALabel(7.23333, 11.9667)[]{\tiny $h_4$}
%
%\FALabel(12.7667, 11.9667)[]{\tiny $h_5$}
%\FALabel(13.9333, 9.63333)[]{\tiny $h_6$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$1^-$}
\FALabel(6.5,16.)[]{\tiny$2^+$}
\FALabel(13.5,16.0)[]{\tiny$3^+$}
\FALabel(17.,4.)[]{\tiny$H$}
%
\end{feynartspicture}

==> DiagramHiggs/C12H.2.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(7.5,15.)(10.0,13.5)(0.,){/Cycles}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(12.5,15.)(10.0,13.5)(0.,){/Cycles}{0}
\FAProp(16.,5.)(13.5,6.5)(0.,){/ScalarDash}{0}
%
% Internal lines
\FAProp(10.0,13.5)(6.5,6.5)(0.,){/ScalarDash}{0}
%\FAProp(13.5,13.5)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){/ScalarDash}{0}
\FAProp(10.0,13.5)(13.5,6.5)(0.,){/ScalarDash}{0}
%
% Vertices 
\FAVert(10.0,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(10.0,13.5){0}
\FAVert(13.5,6.5){0}
%
% Cuts
%\FAProp(15.,10.0)(10.,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.0,10.0)(4.5,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.,15.)(10.0,10.)(0.,){/ScalarDash}{0}
%\FAProp(10.,10.)(10.0,4.5)(0.,){/ScalarDash}{0}
%
% Polarizzazioni
%\FALabel(11.1,4.5)[]{\tiny $h_1$}
%\FALabel(8.9,4.5)[]{\tiny $h_2$}
%\FALabel(5.26667, 10.0333)[]{\tiny $h_3$}
%\FALabel(6.06667, 9.63333)[]{\tiny $h_3$}
%\FALabel(7.23333, 11.9667)[]{\tiny $h_4$}
%
%\FALabel(12.7667, 11.9667)[]{\tiny $h_5$}
%\FALabel(13.9333, 9.63333)[]{\tiny $h_6$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$1^-$}
\FALabel(6.5,16.)[]{\tiny$2^+$}
\FALabel(13.5,16.0)[]{\tiny$3^+$}
\FALabel(17.,4.)[]{\tiny$H$}
%
\end{feynartspicture}

==> DiagramHiggs/C12H3.1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/ScalarDash}{0}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Cycles}{0}
%
% Internal lines
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,13.5)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,13.5)(13.5,6.5)(0.,){/Cycles}{0}
%
% Vertices 
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
%
% Cuts
%\FAProp(15.,10.0)(10.,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.0,10.0)(4.5,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.,15.)(10.0,10.)(0.,){/ScalarDash}{0}
%\FAProp(10.,10.)(10.0,4.5)(0.,){/ScalarDash}{0}
%
% Polarizzazioni
%\FALabel(11.1,4.5)[]{\tiny $h_1$}
%\FALabel(8.9,4.5)[]{\tiny $h_2$}
%\FALabel(4.5, 8.9)[]{\tiny $h_3$}
%\FALabel(4.5, 11.1)[]{\tiny $h_4$}
%\FALabel(8.9, 15.)[]{\tiny $h_5$}
%\FALabel(11.1, 15.)[]{\tiny $h_6$}
%\FALabel(15., 11.1)[]{\tiny $h_7$}
%\FALabel(15., 8.9)[]{\tiny $h_8$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$1^-$}
\FALabel(3.,16.)[]{\tiny$2^+$}
\FALabel(17.,16.)[]{\tiny$H$}
\FALabel(17.,4.)[]{\tiny$3^+$}
%
\end{feynartspicture}


==> DiagramHiggs/C12H3.2.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/ScalarDash}{0}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Cycles}{0}
%
% Internal lines
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/ScalarDash}{0}
\FAProp(13.5,13.5)(6.5,13.5)(0.,){/ScalarDash}{0}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){/ScalarDash}{0}
\FAProp(13.5,13.5)(13.5,6.5)(0.,){/ScalarDash}{0}
%
% Vertices 
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
%
% Cuts
%\FAProp(15.,10.0)(10.,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.0,10.0)(4.5,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.,15.)(10.0,10.)(0.,){/ScalarDash}{0}
%\FAProp(10.,10.)(10.0,4.5)(0.,){/ScalarDash}{0}
%
% Polarizzazioni
%\FALabel(11.1,4.5)[]{\tiny $h_1$}
%\FALabel(8.9,4.5)[]{\tiny $h_2$}
%\FALabel(4.5, 8.9)[]{\tiny $h_3$}
%\FALabel(4.5, 11.1)[]{\tiny $h_4$}
%\FALabel(8.9, 15.)[]{\tiny $h_5$}
%\FALabel(11.1, 15.)[]{\tiny $h_6$}
%\FALabel(15., 11.1)[]{\tiny $h_7$}
%\FALabel(15., 8.9)[]{\tiny $h_8$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$1^-$}
\FALabel(3.,16.)[]{\tiny$2^+$}
\FALabel(17.,16.)[]{\tiny$H$}
\FALabel(17.,4.)[]{\tiny$3^+$}
%
\end{feynartspicture}


==> DiagramHiggs/C1H2.1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(7.5,15.)(10.0,13.5)(0.,){/Cycles}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/ScalarDash}{0}
\FAProp(12.5,15.)(10.0,13.5)(0.,){/Cycles}{0}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Cycles}{0}
%
% Internal lines
\FAProp(10.0,13.5)(6.5,6.5)(0.,){/Cycles}{0}
%\FAProp(13.5,13.5)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(10.0,13.5)(13.5,6.5)(0.,){/Cycles}{0}
%
% Vertices 
\FAVert(10.0,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(10.0,13.5){0}
\FAVert(13.5,6.5){0}
%
% Cuts
%\FAProp(15.,10.0)(10.,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.0,10.0)(4.5,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.,15.)(10.0,10.)(0.,){/ScalarDash}{0}
%\FAProp(10.,10.)(10.0,4.5)(0.,){/ScalarDash}{0}
%
% Polarizzazioni
%\FALabel(11.1,4.5)[]{\tiny $h_1$}
%\FALabel(8.9,4.5)[]{\tiny $h_2$}
%\FALabel(5.26667, 10.0333)[]{\tiny $h_3$}
%\FALabel(6.06667, 9.63333)[]{\tiny $h_3$}
%\FALabel(7.23333, 11.9667)[]{\tiny $h_4$}
%
%\FALabel(12.7667, 11.9667)[]{\tiny $h_5$}
%\FALabel(13.9333, 9.63333)[]{\tiny $h_6$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$H$}
\FALabel(6.5,16.)[]{\tiny$2^+$}
\FALabel(13.5,16.0)[]{\tiny$3^+$}
\FALabel(17.,4.)[]{\tiny$1^-$}
%
\end{feynartspicture}

==> DiagramHiggs/C1H2.2.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(7.5,15.)(10.0,13.5)(0.,){/Cycles}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/ScalarDash}{0}
\FAProp(12.5,15.)(10.0,13.5)(0.,){/Cycles}{0}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Cycles}{0}
%
% Internal lines
\FAProp(10.0,13.5)(6.5,6.5)(0.,){/ScalarDash}{0}
%\FAProp(13.5,13.5)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){/ScalarDash}{0}
\FAProp(10.0,13.5)(13.5,6.5)(0.,){/ScalarDash}{0}
%
% Vertices 
\FAVert(10.0,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(10.0,13.5){0}
\FAVert(13.5,6.5){0}
%
% Cuts
%\FAProp(15.,10.0)(10.,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.0,10.0)(4.5,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.,15.)(10.0,10.)(0.,){/ScalarDash}{0}
%\FAProp(10.,10.)(10.0,4.5)(0.,){/ScalarDash}{0}
%
% Polarizzazioni
%\FALabel(11.1,4.5)[]{\tiny $h_1$}
%\FALabel(8.9,4.5)[]{\tiny $h_2$}
%\FALabel(5.26667, 10.0333)[]{\tiny $h_3$}
%\FALabel(6.06667, 9.63333)[]{\tiny $h_3$}
%\FALabel(7.23333, 11.9667)[]{\tiny $h_4$}
%
%\FALabel(12.7667, 11.9667)[]{\tiny $h_5$}
%\FALabel(13.9333, 9.63333)[]{\tiny $h_6$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$H$}
\FALabel(6.5,16.)[]{\tiny$2^+$}
\FALabel(13.5,16.0)[]{\tiny$3^+$}
\FALabel(17.,4.)[]{\tiny$1^-$}
%
\end{feynartspicture}

==> DiagramHiggs/C1H23.1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/ScalarDash}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Cycles}{0}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Cycles}{0}
%
% Internal lines
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,13.5)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,13.5)(13.5,6.5)(0.,){/Cycles}{0}
%
% Vertices 
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
%
% Cuts
%\FAProp(15.,10.0)(10.,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.0,10.0)(4.5,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.,15.)(10.0,10.)(0.,){/ScalarDash}{0}
%\FAProp(10.,10.)(10.0,4.5)(0.,){/ScalarDash}{0}
%
% Polarizzazioni
%\FALabel(11.1,4.5)[]{\tiny $h_1$}
%\FALabel(8.9,4.5)[]{\tiny $h_2$}
%\FALabel(4.5, 8.9)[]{\tiny $h_3$}
%\FALabel(4.5, 11.1)[]{\tiny $h_4$}
%\FALabel(8.9, 15.)[]{\tiny $h_5$}
%\FALabel(11.1, 15.)[]{\tiny $h_6$}
%\FALabel(15., 11.1)[]{\tiny $h_7$}
%\FALabel(15., 8.9)[]{\tiny $h_8$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$1^-$}
\FALabel(3.,16.)[]{\tiny$H$}
\FALabel(17.,16.)[]{\tiny$2^+$}
\FALabel(17.,4.)[]{\tiny$3^+$}
%
\end{feynartspicture}


==> DiagramHiggs/C1H23.2.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/ScalarDash}{0}
\FAProp(4.,5.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Cycles}{0}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Cycles}{0}
%
% Internal lines
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/ScalarDash}{0}
\FAProp(13.5,13.5)(6.5,13.5)(0.,){/ScalarDash}{0}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){/ScalarDash}{0}
\FAProp(13.5,13.5)(13.5,6.5)(0.,){/ScalarDash}{0}
%
% Vertices 
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
%
% Cuts
%\FAProp(15.,10.0)(10.,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.0,10.0)(4.5,10.0)(0.,){/ScalarDash}{0}
%\FAProp(10.,15.)(10.0,10.)(0.,){/ScalarDash}{0}
%\FAProp(10.,10.)(10.0,4.5)(0.,){/ScalarDash}{0}
%
% Polarizzazioni
%\FALabel(11.1,4.5)[]{\tiny $h_1$}
%\FALabel(8.9,4.5)[]{\tiny $h_2$}
%\FALabel(4.5, 8.9)[]{\tiny $h_3$}
%\FALabel(4.5, 11.1)[]{\tiny $h_4$}
%\FALabel(8.9, 15.)[]{\tiny $h_5$}
%\FALabel(11.1, 15.)[]{\tiny $h_6$}
%\FALabel(15., 11.1)[]{\tiny $h_7$}
%\FALabel(15., 8.9)[]{\tiny $h_8$}
%
% External legs
%
\FALabel(3.,4.)[]{\tiny$1^-$}
\FALabel(3.,16.)[]{\tiny$H$}
\FALabel(17.,16.)[]{\tiny$2^+$}
\FALabel(17.,4.)[]{\tiny$3^+$}
%
\end{feynartspicture}


==> DiagramHiggs/C1H3.1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,11.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(4.,8.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/ScalarDash}{0}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Cycles}{0}
%
% Internal lines
\FAProp(13.5,13.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,13.5)(13.5,6.5)(0.,){/Cycles}{0}
%
% Vertices 
%
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\FAVert(6.5,10.){0}
%
%
% Polarizzazioni
%\FALabel(10.5667, 6.4667)[]{\tiny $h_1$}
%\FALabel(8.23333, 7.6333)[]{\tiny $h_2$}
%\FALabel(8.23333, 12.3667)[]{\tiny $h_3$}
%\FALabel(10.5667, 13.5333)[]{\tiny $h_4$}
%\FALabel(15., 11.1)[]{\tiny $h_5$}
%\FALabel(15., 8.9)[]{\tiny $h_6$}
%
% External legs
%
\FALabel(3.1,8.)[]{\tiny$1^-$}
\FALabel(3.1,12.)[]{\tiny$2^+$}
\FALabel(17.,16.)[]{\tiny$H$}
\FALabel(17.,4.)[]{\tiny$3^+$}
%
\end{feynartspicture}

==> DiagramHiggs/C1H3.2.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,11.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(4.,8.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/ScalarDash}{0}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Cycles}{0}
%
% Internal lines
\FAProp(13.5,13.5)(6.5,10.0)(0.,){/ScalarDash}{0}
\FAProp(6.5,10.0)(13.5,6.5)(0.,){/ScalarDash}{0}
\FAProp(13.5,13.5)(13.5,6.5)(0.,){/ScalarDash}{0}
%
% Vertices 
%
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\FAVert(6.5,10.){0}
%
%
% Polarizzazioni
%\FALabel(10.5667, 6.4667)[]{\tiny $h_1$}
%\FALabel(8.23333, 7.6333)[]{\tiny $h_2$}
%\FALabel(8.23333, 12.3667)[]{\tiny $h_3$}
%\FALabel(10.5667, 13.5333)[]{\tiny $h_4$}
%\FALabel(15., 11.1)[]{\tiny $h_5$}
%\FALabel(15., 8.9)[]{\tiny $h_6$}
%
% External legs
%
\FALabel(3.1,8.)[]{\tiny$1^-$}
\FALabel(3.1,12.)[]{\tiny$2^+$}
\FALabel(17.,16.)[]{\tiny$H$}
\FALabel(17.,4.)[]{\tiny$3^+$}
%
\end{feynartspicture}

==> DiagramHiggs/C23.1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
\FAProp(7.5,15.)(10.0,13.5)(0.,){/Cycles}{0}
\FAProp(12.5,15.)(10.0,13.5)(0.,){/Cycles}{0}
\FAProp(7.5,5.)(10.,6.5)(0.,){/Cycles}{0}
\FAProp(12.5,5.)(10.0,6.5)(0.,){/ScalarDash}{0}
%
\FAVert(10.0,13.5){0}
\FAVert(10.0,6.5){0}
%
\FALabel(6.5,16.)[]{\tiny$3^+$}
\FALabel(13.5,16.0)[]{\tiny$1^-$}
\FALabel(6.5,4.)[]{\tiny$2^+$}
\FALabel(13.5,4.)[]{\tiny$H$}
%
\FAProp(10.0,6.5)(10.0,13.5)(0.8,){/Cycles}{0}
\FAProp(10.0,6.5)(10.0,13.5)(-0.8,){/Cycles}{0}
%
%\FALabel(5.0, 8.9)[]{\tiny $h_1$}
%\FALabel(5.0, 11.1)[]{\tiny $h_2$}
%\FALabel(14.5, 11.1)[]{\tiny $h_3$}
%\FALabel(14.5, 8.9)[]{\tiny $h_4$}
%
\end{feynartspicture}

==> DiagramHiggs/C23.2.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
\FAProp(7.5,15.)(10.0,13.5)(0.,){/Cycles}{0}
\FAProp(12.5,15.)(10.0,13.5)(0.,){/Cycles}{0}
\FAProp(7.5,5.)(10.,6.5)(0.,){/Cycles}{0}
\FAProp(12.5,5.)(10.0,6.5)(0.,){/ScalarDash}{0}
%
\FAVert(10.0,13.5){0}
\FAVert(10.0,6.5){0}
%
\FALabel(6.5,16.)[]{\tiny$3^+$}
\FALabel(13.5,16.0)[]{\tiny$1^-$}
\FALabel(6.5,4.)[]{\tiny$2^+$}
\FALabel(13.5,4.)[]{\tiny$H$}
%
\FAProp(10.0,6.5)(10.0,13.5)(0.8,){/ScalarDash}{0}
\FAProp(10.0,6.5)(10.0,13.5)(-0.8,){/ScalarDash}{0}
%
%\FALabel(5.0, 8.9)[]{\tiny $h_1$}
%\FALabel(5.0, 11.1)[]{\tiny $h_2$}
%\FALabel(14.5, 11.1)[]{\tiny $h_3$}
%\FALabel(14.5, 8.9)[]{\tiny $h_4$}
%
\end{feynartspicture}

==> DiagramHiggs/C23H.1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/ScalarDash}{0}
\FAProp(7.5,5.)(10.,6.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Cycles}{0}
\FAProp(12.5,5.)(10.0,6.5)(0.,){/Cycles}{0}
%
% Internal lines
\FAProp(6.5,13.5)(10.0,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,13.5)(6.5,13.5)(0.,){/Cycles}{0}
%\FAProp(6.5,6.5)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,13.5)(10.0,6.5)(0.,){/Cycles}{0}
%
% Vertices 
%\FAVert(6.5,13.5){0}
\FAVert(6.5,13.5){0}
\FAVert(13.5,13.5){0}
\FAVert(10.0,6.5){0}
%
%
% Polarizzazioni
%\FALabel(11.1,4.5)[]{\tiny $h_1$}
%\FALabel(8.9,4.5)[]{\tiny $h_2$}
%\FALabel(8.9, 15.)[]{\tiny $h_3$}
%\FALabel(11.1, 15.)[]{\tiny $h_4$}
%\FALabel(13.9333, 10.3667)[]{\tiny $h_5$}
%\FALabel(12.7667, 8.03333)[]{\tiny $h_6$}
%
%\FALabel(6.0667, 10.3667)[]{\tiny $h_2$}
%\FALabel(7.2333, 8.03333)[]{\tiny $h_1$}
%
% External legs
%
\FALabel(6.5,4.)[]{\tiny$1^-$}
\FALabel(3.,16.)[]{\tiny$H$}
\FALabel(17.,16.)[]{\tiny$2^+$}
\FALabel(13.5,4.)[]{\tiny$3^+$}
%
\end{feynartspicture}

==> DiagramHiggs/C23H.2.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/ScalarDash}{0}
\FAProp(7.5,5.)(10.,6.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Cycles}{0}
\FAProp(12.5,5.)(10.0,6.5)(0.,){/Cycles}{0}
%
% Internal lines
\FAProp(6.5,13.5)(10.0,6.5)(0.,){/ScalarDash}{0}
\FAProp(13.5,13.5)(6.5,13.5)(0.,){/ScalarDash}{0}
%\FAProp(6.5,6.5)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,13.5)(10.0,6.5)(0.,){/ScalarDash}{0}
%
% Vertices 
%\FAVert(6.5,13.5){0}
\FAVert(6.5,13.5){0}
\FAVert(13.5,13.5){0}
\FAVert(10.0,6.5){0}
%
%
% Polarizzazioni
%\FALabel(11.1,4.5)[]{\tiny $h_1$}
%\FALabel(8.9,4.5)[]{\tiny $h_2$}
%\FALabel(8.9, 15.)[]{\tiny $h_3$}
%\FALabel(11.1, 15.)[]{\tiny $h_4$}
%\FALabel(13.9333, 10.3667)[]{\tiny $h_5$}
%\FALabel(12.7667, 8.03333)[]{\tiny $h_6$}
%
%\FALabel(6.0667, 10.3667)[]{\tiny $h_2$}
%\FALabel(7.2333, 8.03333)[]{\tiny $h_1$}
%
% External legs
%
\FALabel(6.5,4.)[]{\tiny$1^-$}
\FALabel(3.,16.)[]{\tiny$H$}
\FALabel(17.,16.)[]{\tiny$2^+$}
\FALabel(13.5,4.)[]{\tiny$3^+$}
%
\end{feynartspicture}

==> DiagramHiggs/C2H3.1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(7.5,5.)(10.,6.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/ScalarDash}{0}
\FAProp(12.5,5.)(10.0,6.5)(0.,){/Cycles}{0}
%
% Internal lines
\FAProp(6.5,13.5)(10.0,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,13.5)(6.5,13.5)(0.,){/Cycles}{0}
%\FAProp(6.5,6.5)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,13.5)(10.0,6.5)(0.,){/Cycles}{0}
%
% Vertices 
%\FAVert(6.5,13.5){0}
\FAVert(6.5,13.5){0}
\FAVert(13.5,13.5){0}
\FAVert(10.0,6.5){0}
%
%
% Polarizzazioni
%\FALabel(11.1,4.5)[]{\tiny $h_1$}
%\FALabel(8.9,4.5)[]{\tiny $h_2$}
%\FALabel(8.9, 15.)[]{\tiny $h_3$}
%\FALabel(11.1, 15.)[]{\tiny $h_4$}
%\FALabel(13.9333, 10.3667)[]{\tiny $h_5$}
%\FALabel(12.7667, 8.03333)[]{\tiny $h_6$}
%
%\FALabel(6.0667, 10.3667)[]{\tiny $h_2$}
%\FALabel(7.2333, 8.03333)[]{\tiny $h_1$}
%
% External legs
%
\FALabel(6.5,4.)[]{\tiny$1^-$}
\FALabel(3.,16.)[]{\tiny$2^+$}
\FALabel(17.,16.)[]{\tiny$H$}
\FALabel(13.5,4.)[]{\tiny$3^+$}
%
\end{feynartspicture}

==> DiagramHiggs/C2H3.2.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,15.)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(7.5,5.)(10.,6.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/ScalarDash}{0}
\FAProp(12.5,5.)(10.0,6.5)(0.,){/Cycles}{0}
%
% Internal lines
\FAProp(6.5,13.5)(10.0,6.5)(0.,){/ScalarDash}{0}
\FAProp(13.5,13.5)(6.5,13.5)(0.,){/ScalarDash}{0}
%\FAProp(6.5,6.5)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,13.5)(10.0,6.5)(0.,){/ScalarDash}{0}
%
% Vertices 
%\FAVert(6.5,13.5){0}
\FAVert(6.5,13.5){0}
\FAVert(13.5,13.5){0}
\FAVert(10.0,6.5){0}
%
%
% Polarizzazioni
%\FALabel(11.1,4.5)[]{\tiny $h_1$}
%\FALabel(8.9,4.5)[]{\tiny $h_2$}
%\FALabel(8.9, 15.)[]{\tiny $h_3$}
%\FALabel(11.1, 15.)[]{\tiny $h_4$}
%\FALabel(13.9333, 10.3667)[]{\tiny $h_5$}
%\FALabel(12.7667, 8.03333)[]{\tiny $h_6$}
%
%\FALabel(6.0667, 10.3667)[]{\tiny $h_2$}
%\FALabel(7.2333, 8.03333)[]{\tiny $h_1$}
%
% External legs
%
\FALabel(6.5,4.)[]{\tiny$1^-$}
\FALabel(3.,16.)[]{\tiny$2^+$}
\FALabel(17.,16.)[]{\tiny$H$}
\FALabel(13.5,4.)[]{\tiny$3^+$}
%
\end{feynartspicture}

==> FeynmanDiagrams/5gT1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(0.,17.)(7.,13.5)(0.,){/Cycles}{0}
\FAProp(0.,10.)(7.,6.5)(0.,){/Cycles}{0}
\FAProp(0.,3.)(7.,6.5)(0.,){/Cycles}{0}
\FAProp(20.,15.)(13.,10.)(0.,){/Cycles}{0}
\FAProp(20.,5.)(13.,10.)(0.,){/Cycles}{0}
\FAProp(7.,13.5)(7.,6.5)(0.,){/Cycles}{0}
\FAProp(7.,13.5)(13.,10.)(0.,){/Cycles}{0}
\FAProp(7.,6.5)(13.,10.)(0.,){/Cycles}{0}
%
% Vertices 
\FAVert(7.,13.5){0}
\FAVert(7.,6.5){0}
\FAVert(13.,10.){0}
%
% Label for particles
%
%\FALabel(3.60138,15.9328)[r]{$1$}
%\FALabel(3.39862,7.56724)[br]{$2$}
%\FALabel(3.60138,4.06724)[r]{$3$}
%\FALabel(16.7756,11.9221)[r]{$4$}
%\FALabel(16.2244,6.92215)[r]{$5$}
%
\end{feynartspicture}

==> FeynmanDiagrams/5sD.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(0.,17.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,10.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,3.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(14.,10.)(0.,){/Cycles}{0}
\FAProp(20.,5.)(14.,10.)(0.,){/Cycles}{0}
\FAProp(14.,10.)(6.,10.)(0.8,){/ScalarDash}{0}
\FAProp(14.,10.)(6.,10.)(-0.8,){/ScalarDash}{0}
%
% Vertices 
\FAVert(14.,10.){0}
\FAVert(6.,10.){0}
%
% Label for particles
%
\FALabel(2.49297,13.134)[r]{$1$}
\FALabel(3.,9.18)[r]{$2$}
\FALabel(3.50703,6.13397)[r]{$3$}
\FALabel(16.6478,13.0187)[l]{$4$}
\FALabel(17.3522,8.01869)[l]{$5$}
%
\end{feynartspicture}

==> FeynmanDiagrams/5sT1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(0.,17.)(7.,13.5)(0.,){/Cycles}{0}
\FAProp(0.,10.)(7.,6.5)(0.,){/Cycles}{0}
\FAProp(0.,3.)(7.,6.5)(0.,){/Cycles}{0}
\FAProp(20.,15.)(13.,10.)(0.,){/Cycles}{0}
\FAProp(20.,5.)(13.,10.)(0.,){/Cycles}{0}
\FAProp(7.,13.5)(7.,6.5)(0.,){/ScalarDash}{0}
\FAProp(7.,13.5)(13.,10.)(0.,){/ScalarDash}{0}
\FAProp(7.,6.5)(13.,10.)(0.,){/ScalarDash}{0}
%
% Vertices 
\FAVert(7.,13.5){0}
\FAVert(7.,6.5){0}
\FAVert(13.,10.){0}
%
% Label for particles
%
\FALabel(3.60138,15.9328)[r]{$1$}
\FALabel(3.39862,7.56724)[br]{$2$}
\FALabel(3.60138,4.06724)[r]{$3$}
\FALabel(16.7756,11.9221)[r]{$4$}
\FALabel(16.2244,6.92215)[r]{$5$}
%
\end{feynartspicture}

==> FeynmanDiagrams/5sT2.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(0.,17.)(10.,12.5)(0.,){/Cycles}{0}
\FAProp(0.,10.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(0.,3.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,12.5)(0.,){/Cycles}{0}
\FAProp(20.,5.)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,6.5)(10.,12.5)(0.,){/ScalarDash}{0}
\FAProp(13.5,6.5)(6.5,6.5)(0.,){/ScalarDash}{0}
\FAProp(10.,12.5)(6.5,6.5)(0.,){/ScalarDash}{0}
%
% Vertices 
\FAVert(13.5,6.5){0}
\FAVert(10.,12.5){0}
\FAVert(6.5,6.5){0}
%
% Label for particles
%
\FALabel(4.94653,14.0445)[r]{$1$}
\FALabel(3.11367,7.58539)[r]{$2$}
\FALabel(3.38633,4.08539)[r]{$3$}
\FALabel(14.6847,14.5312)[l]{$4$}
\FALabel(16.4577,4.96329)[l]{$5$}
%
\end{feynartspicture}

==> FeynmanDiagrams/5sT3.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(0.,17.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,10.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,3.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(14.,12.)(0.,){/Cycles}{0}
\FAProp(20.,5.)(14.,8.)(0.,){/Cycles}{0}
\FAProp(14.,12.)(14.,8.)(0.,){/ScalarDash}{0}
\FAProp(14.,12.)(6.,10.)(0.,){/ScalarDash}{0}
\FAProp(14.,8.)(6.,10.)(0.,){/ScalarDash}{0}
%
% Vertices 
\FAVert(14.,12.){0}
\FAVert(14.,8.){0}
\FAVert(6.,10.){0}
%
% Label for particles
%
\FALabel(2.49297,13.134)[r]{$1$}
\FALabel(3.,9.18)[r]{$2$}
\FALabel(3.50703,6.13397)[r]{$3$}
\FALabel(16.8986,14.1828)[l]{$4$}
\FALabel(17.1014,7.18276)[l]{$5$}
%
\end{feynartspicture}

==> FeynmanRules/FF.tex <==
\unitlength=0.20bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(4.,10.)(16.,10.)(0.,){/Straight}{1}
\FALabel(5.5,8.93)[t]{\tiny $i$}
\FALabel(14.5,8.93)[t]{\tiny $j$}
\FALabel(10.,12.5)[]{\tiny $k$}
\FAVert(4.,10.){0}
\FAVert(16.,10.){0}
\end{feynartspicture}

==> FeynmanRules/FFG.tex <==
\unitlength=0.20bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(3.,10.)(10.,10.)(0.,){/Straight}{1}
\FALabel(5.3,8.93)[t]{\tiny $1, i$}
\FAProp(16.,15.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(12.2273,13.5749)[br]{\tiny $2, b, \beta$}
\FAProp(16.,5.)(10.,10.)(0.,){/Straight}{-1}
\FALabel(12.8873,5.81315)[tr]{\tiny $3, j$}
\FAVert(10.,10.){0}
\end{feynartspicture}

==> FeynmanRules/FFS.tex <==
\unitlength=0.20bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(3.,10.)(10.,10.)(0.,){/Straight}{1}
\FALabel(5.3,8.93)[t]{\tiny $1, i$}
\FAProp(16.,15.)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(12.2273,13.5749)[br]{\tiny $2, b, B$}
\FAProp(16.,5.)(10.,10.)(0.,){/Straight}{-1}
\FALabel(12.8873,5.81315)[tr]{\tiny $3, j$}
\FAVert(10.,10.){0}
\end{feynartspicture}

==> FeynmanRules/GG.tex <==
\unitlength=0.20bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(4.,10.)(16.,10.)(0.,){/Cycles}{0}
\FALabel(5.5,8.93)[t]{\tiny $a, \alpha$}
\FALabel(14.5,8.93)[t]{\tiny $b, \beta$}
\FALabel(10.,12.5)[]{\tiny $k$}
\FAVert(4.,10.){0}
\FAVert(16.,10.){0}
\end{feynartspicture}

==> FeynmanRules/GGG.tex <==
\unitlength=0.20bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(3.,10.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(5.3,8.93)[t]{\tiny $1, a, \alpha$}
\FAProp(16.,15.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(12.2273,13.5749)[br]{\tiny $2, b, \beta$}
\FAProp(16.,5.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(12.8873,5.81315)[tr]{\tiny $3, c, \gamma$}
\FAVert(10.,10.){0}
\end{feynartspicture}

==> FeynmanRules/GGGG.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(4.,15.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(3.0,12.)[]{\tiny $1,a,\alpha$}
\FAProp(10.,10.)(4.,5.)(0.,){/Cycles}{0}
\FALabel(3.0,8.)[]{\tiny $4,d,\delta$}
\FAProp(16.,15.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(11.,15.)[]{\tiny $2,b,\beta$}
\FAProp(10.,10.)(16.,5.)(0.,){/Cycles}{0}
\FALabel(11,5.)[]{\tiny $3,c,\gamma$}
\FAVert(10.,10.){0}
\end{feynartspicture}

==> FeynmanRules/GGS.tex <==
\unitlength=0.20bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(3.,10.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(5.3,8.93)[t]{\tiny $1, a, \alpha$}
\FAProp(16.,15.)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(12.2273,13.5749)[br]{\tiny $2, b, B$}
\FAProp(16.,5.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(12.8873,5.81315)[tr]{\tiny $3, c, \gamma$}
\FAVert(10.,10.){0}
\end{feynartspicture}

==> FeynmanRules/GGS_copy.tex <==
\unitlength=0.20bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(3.,10.)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(5.3,8.93)[t]{\tiny $1, a, A$}
%\FALabel(5.5,8.93)[t]{\tiny $1, a, A$}
\FAProp(16.,15.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(12.2273,13.5749)[br]{\tiny $2, b, \beta$}
\FAProp(16.,5.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(12.8873,5.81315)[tr]{\tiny $3, c, \gamma$}
\FAVert(10.,10.){0}
\end{feynartspicture}

==> FeynmanRules/GSS.tex <==
\unitlength=0.20bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(3.,10.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(5.3,8.93)[t]{\tiny $1,a, \alpha$}
\FAProp(16.,15.)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(12.2273,13.5749)[br]{\tiny $2, b, B$}
\FAProp(16.,5.)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(12.8873,5.81315)[tr]{\tiny $3,c, C$}
\FAVert(10.,10.){0}
\end{feynartspicture}

==> FeynmanRules/P3.tex <==
\unitlength=0.20bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(3.,10.)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(5.5,8.93)[t]{\tiny $a, A$}
\FAProp(16.,15.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(12.2273,13.3749)[br]{\tiny $b, \beta$}
\FAProp(16.,5.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(12.8873,6.01315)[tr]{\tiny $c, \gamma$}
\FAVert(10.,10.){0}
\end{feynartspicture}

==> FeynmanRules/P4.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(4.,15.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(3.0,13.)[]{\tiny $1,a,\alpha$}
\FAProp(4.,5.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(3.0,7.)[]{\tiny $4,d,\delta$}
\FAProp(16.,15.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(14.7868,13.4064)[]{\tiny $g_1$}
\FAProp(16.,5.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(15.2132,8.40636)[]{\tiny $g_2$}
\FAVert(10.,10.){0}
\end{feynartspicture}

==> FeynmanRules/PRO.1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
\FAProp(4.,10.0)(6.5,10.0)(0.,){/Straight}{1}
\FAProp(1.,10.0)(4.,10.0)(0.,){/GhostDash}{0}
\FAProp(16.,10.0)(13.5,10.0)(0.,){/Straight}{-1}
\FAProp(16.,10.0)(19.0,10.0)(0.,){/GhostDash}{0}
%
\FAVert(6.5,10.){0}
\FAVert(13.5,10.0){0}
%
\FAProp(6.5,10.)(13.5,10.0)(0.8,){/Straight}{1}
\FAProp(6.5,10.)(13.5,10.0)(-0.8,){/Cycles}{0}
\FALabel(10.0,5.5)[]{\tiny $\bar \ell$}
%
\end{feynartspicture}

==> FeynmanRules/PRO.2.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,11.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(4.,8.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(13.5,13.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,6.5)(13.5,13.5)(0.,){/Straight}{-1}
%
% Vertices 
%
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\FAVert(6.5,10.){0}
%
\FAProp(4.,11.5)(1.5,13.0)(0.,){/GhostDash}{0}
\FAProp(4.,8.5)(1.5,7.0)(0.,){/GhostDash}{0}
\FAProp(16.,15.)(18.5, 16.5)(0.,){/GhostDash}{0}
\FAProp(16.,5.)(18.5, 3.5)(0.,){/GhostDash}{0}
%
%
\end{feynartspicture}

==> FeynmanRules/PRO.3.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
%\FAProp(4.,11.5)(6.5,10.0)(0.,){/Cycles}{0}
%\FAProp(6.5,10.0)(4.,8.5)(0.,){/Cycles}{0}
\FAProp(3.5,10.0)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(1.,10.0)(3.5,10.0)(0.,){/GhostDash}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(13.5,13.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,6.5)(13.5,13.5)(0.,){/Straight}{-1}
\FALabel(14.8,10.0)[]{\tiny $\bar \ell$}
%
% Vertices 
%
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\FAVert(6.5,10.){0}
%
%\FAProp(4.,11.5)(1.5,13.0)(0.,){/GhostDash}{0}
%\FAProp(4.,8.5)(1.5,7.0)(0.,){/GhostDash}{0}
\FAProp(16.,15.)(18.5, 16.5)(0.,){/GhostDash}{0}
\FAProp(16.,5.)(18.5, 3.5)(0.,){/GhostDash}{0}
%
%
\end{feynartspicture}

==> FeynmanRules/PRO.4.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
%\FAProp(4.,11.5)(6.5,10.0)(0.,){/Cycles}{0}
%\FAProp(6.5,10.0)(4.,8.5)(0.,){/Cycles}{0}
\FAProp(3.5,10.0)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(1.,10.0)(3.5,10.0)(0.,){/GhostDash}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(13.5,13.5)(6.5,10.0)(0.,){/Straight}{1}
\FAProp(6.5,10.0)(13.5,6.5)(0.,){/Straight}{1}
\FAProp(13.5,6.5)(13.5,13.5)(0.,){/Cycles}{0}
%
% Vertices 
%
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\FAVert(6.5,10.){0}
%
%\FAProp(4.,11.5)(1.5,13.0)(0.,){/GhostDash}{0}
%\FAProp(4.,8.5)(1.5,7.0)(0.,){/GhostDash}{0}
\FAProp(16.,15.)(18.5, 16.5)(0.,){/GhostDash}{0}
\FAProp(16.,5.)(18.5, 3.5)(0.,){/GhostDash}{0}
%
\FALabel(9.5,14.0)[]{\tiny $\bar \ell +p$}
\FALabel(10.0,6.0)[]{\tiny $\bar \ell$}
%
\end{feynartspicture}

==> FeynmanRules/SS.tex <==
\unitlength=0.20bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(4.,10.)(16.,10.)(0.,){/ScalarDash}{0}
\FALabel(5.5,8.93)[t]{\tiny $a, A$}
\FALabel(14.5,8.93)[t]{\tiny $b, B$}
\FALabel(10.,12.5)[]{\tiny $k$}
\FAVert(4.,10.){0}
\FAVert(16.,10.){0}
\end{feynartspicture}

==> FeynmanRules/SSGG.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(4.,15.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(3.0,12.)[]{\tiny $1,a,\alpha$}
\FAProp(10.,10.)(4.,5.)(0.,){/Cycles}{0}
\FALabel(3.0,8.)[]{\tiny $4,d,\delta$}
\FAProp(16.,15.)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(11.,15.)[]{\tiny $2,b,B$}
\FAProp(10.,10.)(16.,5.)(0.,){/ScalarDash}{0}
\FALabel(11,5.)[]{\tiny $3,c,C$}
\FAVert(10.,10.){0}
\end{feynartspicture}

==> FeynmanRules/gogo.tex <==
\unitlength=0.20bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(4.,10.)(16.,10.)(0.,){/GhostDash}{1}
\FALabel(5.5,8.93)[t]{\tiny $a$}
\FALabel(14.5,8.93)[t]{\tiny $b$}
\FALabel(10.,12.5)[]{\tiny $k$}
\FAVert(4.,10.){0}
\FAVert(16.,10.){0}
\end{feynartspicture}

==> FeynmanRules/gogoG.tex <==
\unitlength=0.20bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(3.,10.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(5.3,8.93)[t]{\tiny $1, a, \alpha$}
\FAProp(16.,15.)(10.,10.)(0.,){/GhostDash}{-1}
\FALabel(12.2273,13.5749)[br]{\tiny $2, b$}
\FAProp(16.,5.)(10.,10.)(0.,){/GhostDash}{1}
\FALabel(12.8873,5.81315)[tr]{\tiny $3, c$}
\FAVert(10.,10.){0}
\end{feynartspicture}
